Folding interpretations

We study the polyregular string-to-string functions, which are certain functions of polynomial output size that can be described using automata and logic. We describe a system of combinators that generates exactly these functions. Unlike previous systems, the present system includes an iteration mechanism, namely fold. Although unrestricted fold can define all primitive recursive functions, we identify a type system (inspired by linear logic) that restricts fold so that it defines exactly the polyregular functions. We also present related systems, for quantifier-free functions as well as for linear regular functions on both strings and trees.

==> ap-poly-complete.tex <==
\section{Completeness of the system}


==> derivable-are-polyregular.tex <==
\subsection{Weakly derivable functions are polyregular}


Let $\tau$ and $\sigma$ be classes of graded structures. A function 
\begin{align*}
f : \tau \to \sigma
\end{align*}
is called an \emph{$\ell$-downgrading interpretation} if for every input $A \in \tau$, all of the following conditions are satisfied:
\begin{enumerate}
\item The output $f(A)$ contains $A$,  which means that $A$ can be  obtained from $f(A)$ by restricting its universe to some subset of elements.
\item The \emph{new output elements} of $f(A)$, i.e.~the elements of $f(A)$ that are  not in $A$, all have grade $\ell$. 
\item If a relation in $f(A)$  selects a tuple that contains some new output elements, then all other elements in the tuple are either new output elements or have grade at least $\ell+1$.
\item The following function is polyregular, once the grades are ignored:
\begin{align*}
A | \text{(grade $> \ell$)} \quad \mapsto \quad f(A)|\text{(new or grade $> \ell$)}
\end{align*}
\end{enumerate}


\begin{myexample}
    Suppose that $f : \tau \to \sigma$ is a polyregular function where both input and output types are  !-free. Then the function of type $!\tau \to \sigma$ defined by 
    \begin{align*}
    !A \quad \mapsto \quad f(A)
    \end{align*}
    is a 1-downgrading polyregular function.  
\end{myexample}
\begin{definition}
    A \emph{graded polyregular function} is any finite composition of functions that are either quantifier-free interpretations, or $\ell$-downgrading polyregular for some $\ell$. 
\end{definition}

\begin{definition}
    A \emph{graded \mso interpretation} is defined as follows. The syntax is the same as that of  an \mso interpretation (see Definition~\ref{def:mso-interpretation}), plus:
    \begin{itemize}
        \item for each component, there is an associated  \emph{grade} in $\set{0,1,\ldots}$;
        \item for each grade, there is a  distinguished \emph{equi-graded} component of this grade, which has dimension one.
    \end{itemize}
      The output structure is defined in the same way as for  \mso interpretations, with the grade of elements from component $q$ being equal to the grade of $q$.  Furthermore, the  interpretation must satisfy the following conditions:
    \begin{enumerate}
        \item Let $q$ be a component of grade $\ell$. If
        \begin{align*}
        q(\bar a) \in f(A),
        \end{align*}
        then: if $q$ is equi-graded, then the unique element in $\bar a$ (it is unique because the equi-graded components have dimension one) has the same grade as $q$; otherwise all elements in $\bar a$ have grade strictly bigger than $q$.
        \item For every component $q$ there is some  quantifier rank $r \in \set{0,1,\ldots}$ such that whether or not
        \begin{align*}
        q(\bar a) \in f(A)
        \end{align*}
         depends only on  the following two types:
            \begin{align*}
            \text{rank $r$ type of } & (A, \bar a)|1 + \text{grade of $q$}\\
            \text{quantifier free type of } & (A, \bar a)|\text{grade of $q$}
            \end{align*}
    

        \item Let $R$ be an $m$-ary relation of the output vocabulary, and let  $q_1,\ldots,q_m$ be components. There is some quantifier rank $r \in \set{0,1,\ldots}$ such that   whether or not 
        \begin{align*}
        f(A) \models R(q_1(\bar a_1),\ldots, q_m(\bar a_m))
        \end{align*}
        depends only on the following two types:
            \begin{align*}
            \text{rank $r$ type of } & (A, \bar a_1,\ldots \bar a_m)|1 + \text{minimal grade in $\bar q$}\\
            \text{quantifier free type of } & (A, \bar a_1,\ldots \bar a_m)|\text{minimal grade in $\bar q$}
            \end{align*}
    
        
    \end{enumerate}
\end{definition}



For graded datatypes $\tau$ and $\sigma$, a function of type $f : \tau \to \sigma$ is called \emph{graded polyregular} if it is a function between the corresponding classes of graded structures that is defined by a graded \mso interpretation. 

\begin{lemma}
    The graded polyregular functions contain all functions in Figure~\ref{fig:prime-poly}, and are closed under the combinators in Figure~\ref{fig:comb-poly}.
\end{lemma}
\begin{proof}
    With one exception, all of the functions in Figure~\ref{fig:prime-poly} are quantifier-free interpretations that do not change the grades, and  such functions are clearly graded polyregular. The one exception is the  copying function
    \begin{align*}
    \upgrade \tau \to \upgrade \tau \times \tau,
    \end{align*}
    which is easily seen to be graded polyregular (there are down-graded copy names of arity one that are used to create the down-graded copy of $\tau$).
     
    We are left with the combinators. The functoriality combinators are easily seen to preserve graded polyregular functions. The composition combinator is also not hard, one we know that that \mso interpretations are closed under composition over datatypes. The remaining case is fold. 

    
\end{proof}

\input{new-proof}


\begin{lemma}
    If $\Aa : \sigma + \tau \times \sigma \to \tau$ is graded polyregular, then the same is true for its fold.
\end{lemma}
\begin{proof}
    Consider an input to the fold, which is of the form 
    \begin{align*}
   A =  \upgrade{[A_1,\ldots,A_n]} \in \upgrade{(\tau^+)}
    \end{align*}
    Throughout the proof, we will use the notation that 
    \begin{align*}
    B = [B_1,\ldots,B_n]
    \end{align*}
    is the list where $B_i$  is the fold applied to the first $i$ elements of $A$. For $\ell \in \set{0,1,\ldots}$, define $B_i | \ell$ to be the structure that is obtained from $B_i$ by keeping only the elements of grade at least $\ell$.  We will also consider intermediate values: define $B_i | \ell + \half$ to be the structure $B_i$ which is obtained from $B_i$ by restricting the universe to elements that have either grade at least $\ell+1$, or have grade exactly $\ell$ and were down-graded when $B_i$ was created.  (If $i=1$ then $B_i$ is created by applying the intial function of $\Aa$ to $A_i$, and if $i > i$ then $B_{i}$ is created by applying the update function to $B_{i-1}$ and $A_i$.) These structures are ordered by inclusion (i.e.~one is an induced structure of the other) as follows:
    \begin{align*}
    B_i = B_i| 0 \quad \supseteq \quad 
    B_i|\tfrac 1 2 \quad \supseteq \quad 
    B_i|1 \quad \supseteq \quad 
    B_i|1+\tfrac 1 2 \quad  \supseteq \cdots
    \end{align*}
    Also, $B_i | \ell$ is empty whenever $\ell$ is exceeds the maximal grade in the graded datatype $\tau$. 
    The main step in the proof is the following claim, which shows that the above restrictions of the output structures can be computed by a graded polyregular function. 
    

    \begin{claim}
        For every $\ell \in \set{0,\half, 1, 1 \half, 2, \ldots}$, the following function, call it $f_\ell$, is graded polyregular
        \begin{gather*}
            [!A_1,\ldots,!A_n] \\
            \downmapsto \\ 
            [(! A_1, B_1|\ell), \ldots, (!A_n, B_n |\ell)].
        \end{gather*}     
    \end{claim}
    \begin{proof}
        The proof is a backward induction on $\ell$. 
        In the induction step, we  show that the output of $f_\ell$ can be computed once we know the output of $f_{\ell+\half}$.  This induction is well-founded, since whenever $\ell$ exceeds the maximal grade of elements in the type $\tau$, then $f_{\ell}$ is simply the identity function, which is clearly graded polyregular. 
        There are two cases, for the induction step,  depending on whether the index $\ell$ is an integer or fractional.


        \paragraph*{Fractional index.}
        Consider a fractional index of the form $\ell + \half$ with $\ell \in \set{0,1,\ldots}$. By induction assumption, we can use a graded polyregular function to compute 
        \begin{align*}
        [(!A,B_1|\ell+1), \ldots, (!A,B_n|\ell+1)].
        \end{align*}
        Because the state update function is graded polyregular, it follows that  for $i > 1$, the structure $B_i | \ell + \half$ can be obtained by applying a graded polyregular function to the pair 
        \begin{align*}
        (B_{i-1}| \ell + 1, A_i | \ell+1),
        \end{align*} 
        and this pair is known thanks to the .

        
          


        \paragraph*{Integer indices.} Consider an integer index  $\ell \in \set{0,1,\ldots}$. We will show that the output of $f_{\ell}$ can be computed once we know the output of $f_{\ell + \half}$. Here, we use the same proof as in Theorem~\ref{thm:fold-quantifier-free}. Define the new elements in the same way as in the fractional case: these are the elements of the output of $f_{\ell}$ that are not already in the output of $f_{\ell+\half}$.  All new elements are equi-graded. By definition of polyregular functions and equi-graded elements, it follows that if $b \in B_i$ is new, then it is either an element of grade $\ell$ in 
        Consider first the case when $\ell$ is an integer in $\set{0,1,\ldots}$. By definition of graded polyregular functions, elements the map 
        \begin{align*}
        (B_i|\ell+\half, A_i) \quad \mapsto \quad B_i|\ell
        \end{align*}
        
        
        If $\ell$ exceeds the maximal grade of elements in $\tau$, then there is nothing to do, since the structures $B_i|\ell$ will all be empty, so the function $f_\ell$ is simply the identity. To get the result of the claim  smaller $\ell$, we will show that the function 
        \begin{align}\label{eq:one-step-fl}
        f_{\ell+1}(A) \quad \mapsto \quad f_{\ell}(A)
        \end{align}
        is graded polyregular. By composing functions as in~\eqref{eq:one-step-fl}, we get the function from the statement of the claim. It remains to prove that the function~\eqref{eq:one-step-fl} is  graded polyregular. Suppose that we are given the input structure, i.e.~we are given 
        \begin{align*}
        f_{\ell+1}(A) = [(! A_1, B_1|\ell+1), \ldots, (!A_n, B_n |\ell+1)].
        \end{align*}
        We now want to compute, using a graded polyregular function, the structure $f_{\ell}(A)$. There are two kinds of elements in  this structure
        \begin{itemize}
        \item[(a)]the elements of the input structure; and
        \item[(b)] elements of grade exactly $\ell$ in the structures $B_1,\ldots,B_\ell$
        \end{itemize}
        Furthermore, on elements of the first kind, the relations are defined in the same way as in the input, i.e.~the input structure $f_{\ell+1}(A)$ is an induced substructure of $f_{\ell}(A)$. Therefore, it remains to define the elements of kind (b), and how they relate to other elements of kinds (a) and (b). Elements of kind (b) can be further classified into two sub-kinds: down-graded, or equi-graded, depending on whether they were down-graded or equi-graded when they were created. (Elements of $B_1$ are created when applying the initial function of the automaton to $A_1$, while elements of $B_{i}$ with $i > 1$ are created when applying the transition function to the pair $B_{i-1}$ and $A_i$.) 

        We first define the down-graded elements. Define $f_{\ell + \half}(A)$ to be the structure which is obtained from $f_{\ell}(A)$ be restricting the elements of kind (b) to the down-graded ones. 

        
    \end{proof}
    
    The proof is by  induction, but in the opposite order: from bigger numbers  $\ell$ down to smaller ones. 
    
    If $\bar a$ is a tuple of elements in $(B_i,A_i)$ and $b$ is an element of $B_{i+1}$, and $c$ is a component of the transduction $\delta$, then we write 
    In the proof, we will be working in the disjoint union of all the input letters and states, i.e.~the set of elements
    \begin{align*}
    C = A_1 + \cdots + A_n + B_1 + \cdots + B_n.
    \end{align*}
    An element of $C$ is either of the form $a \in A_i$ for some $i \in \set{1,\ldots,n}$, or of the form $b \in B_i$.  We define two relations on $C$. The \emph{equi-graded} 


    For an element $b \in B_i$ define its \emph{origin tree} as follows. Let the origin of $b$ be 
    \begin{align*}
    q(c_1,\ldots,c_n) 
    \end{align*}
    with $c_1,\ldots,c_n$ being elements of the pair structure $(B_i,A_i)$. By definition of the pair structure, each of the elements of $c_1,\ldots,c_n$ is either in $B_i$ or in $A_i$. The origin tree of $b$ is defined to be the tree which has $q$ in the root, and $n$ children, consisting of the origin trees of the elements $c_1,\ldots,c_n$. Define the \emph{origin tree structure} (for the input $A$) to be the following structure, which will be denoted by $T(A)$. It consists of the disjoint union of the structure $A$ with the set of all origin trees, together with the following extra predicates:
    \begin{itemize}
    \item A binary predicate which selects all pairs $(a,t)$ such that for some $i \in \set{1,\ldots,n}$, $a$ belongs to $a_i$ and $t$ is the origin tree of some element in $B_i$. 
    \item For every relation $R(y_1,\ldots,y_m)$ in the vocabulary of $\tau$, a relation with the same name that  consists of tuples which can be obtained by choosing some $i \in \set{1,\ldots,n}$, choosing some tuple $\bar b$ in the interpretation of $R$ in $B_i$, and returning the tuples of origin trees of elements in $\bar b$. 
    There is a binary predicate for the subtree relation on origin trees, and for every $i \in \set{1,\ldots,k}$ a binary predicate for the $i$-th child relation. 
    \item For every relation name $R$ in the input vocabulary 
    \end{itemize}

    Define a \emph{derivation} to be a tree where: non-leaf nodes are components of the transition function, leaf nodes are labelled by elements of $A$, and if a non-leaf node is labelled by a component $c$, then it has exactly $k(c)$ children, which are labelled by components of grade strictly bigger than the grade of $c$. Since the grades must strictly increase in a derivation along every root-to-leaf path, and the number of children is bounded, the number of leaves in a derivation.

    \begin{claim}
        For every relation $R(y_1,\ldots,y_n)$ of the vocabulary of $\tau$, 
        For every derivation shape $t$ with there is an 
    \end{claim}

    For each element $c \in T$, we define a \emph{derivation}, which is a tree of the following form: non-leaf nodes of the tree are labelled by components, leaves are labelled by 
    We define a directed acyclic graph on $C$ as follows. 
    
    \begin{align*}
    \alpha : X \to 1 + X + \coprod_{c \in C} X^{k(c)}
    \end{align*}
    The leaves of this tree are the elements of the letter structures $A_1,\ldots,A_n$. If $c$ is not 

    For $c \in C$, define its \emph{progenitor} to be the the unique equi-graded ancestor $d \in C$ of $c$ such that either $d$ is an element of one of the input letters $A_1,\ldots,A_n$, or $d$ is a down-graded element of some $B_i$, 

    We say that $b \in B_i$ is the \emph{equi-grade parent} of $b' \in B_{i+1}$ if (..).  We say that $b \in B_i$ is an \emph{equi-grade ancestor} of $b' \in B_{j}$ if one can go from $b'$ to 

    Define the \emph{ancestor} of 
\end{proof}
The trees in this section will have constant depth, all leaves will be sibling-ordered (i.e.~for each node its children have a total order), and labelled with the following alphabet: 
\begin{align*}
    \myunderbrace{\times}{arity two} \qquad 
\myunderbrace{\upgrade{\ }  \qquad \leftinj \qquad \rightinj}{arity one}   
\qquad  \myunderbrace 1 {arity zero} \qquad 
\myunderbrace{*}{no arity}.
\end{align*}
The arities indicate the number of children: a node with arity two has exactly two children, likewise for arities one and zero. The label $*$ has no arity, which means that a node with label $*$ can have any number of children in $\set{0,1,\ldots}$. Here is a picture of such a tree:
\begin{center}
    ..
\end{center}

For a datatype $\tau$, we define its \emph{tree representation}, denoted by $\trees \tau$,  to be the set of trees that corresponds to $\tau$, which is defined in the natural way and illustrated in the following example of a tree in the tree representation of the type 
\begin{align*}
 \tau = ...
\end{align*} 

We will transform tree representations into other tree representations using \mso interpretations. To this end, we will need to represent trees as models. Since we will also want to use quantifier-free interpretations, the choice of relations in the vocabulary will be important. 

For a tree $t$, we say that a node $y$ is \emph{visible} from $x$ if one can go from $x$ to $y$ by a finite (possibly zero) number of steps of the following forms: ``go to the parent'' or  ``go to a child of a node with label other than $*$''.  If the depth of the tree is constant, then the number of visible nodes is also constants: if the tree has depth at most $k$, then there are at most $2^k$ nodes  are visible for any given node. For a tree $t$ with distinguished nodes $x_1,\ldots,x_n$ is defined  to be the tree that is obtained from $t$ by keeping only the nodes $x_1,\ldots,x_n$ and the nodes visible from them. The number of possible profiles is bounded by a function of the depth of the tree and the number of distinguished nodes. We also care about the profile of a tree with $n=0$ distinguished nodes, in this case we restrict the tree to nodes that are visible from the root.

\begin{definition}
    Consider a datatype $\tau$ and a  tree $t \in \trees \tau$. The  \emph{model}  of $t$ is defined as follows. The universe  of the model consists of the leaves in $t$ that have  label $1$. For every $i \in \set{0,1,2}$ and every possible profile $p$ that can arise in a tree from $\trees \tau$ with $i$ distinguished nodes, there is a predicate $p(x_1,\ldots,x_i)$ which selects $i$-tuples of nodes that have profile $p$. (When $i=0$, the predicate is Boolean, i.e.~it takes no arguments and has value ``true'' or ``false''.)
\end{definition}


For a tree $t \in \trees(\tau)$, its \emph{strength} is defined to be the number of ancestors that have the strengthening label $\upgrade {}$. We define $t | i$ to be the model that is obtained from the model of $t$ and restricting its universe to  leaves that have strength at least $i$, and nodes that are visible from them.

Consider two graded datatypes $\tau$ and $\sigma$. We say that  a function $ f  : \tau \to \sigma$ 
is  \emph{graded polyregular} if for every $i \in \set{0,1,\ldots}$ there is some graded datatype $\rho_i$ and functions   
\begin{align*}
f_i  & : \restrictmore \tau i  \to \rho_i \\
g_i  & : \rho_i \times \restrict \tau i  \to \restrict \sigma i
\end{align*}
with $f_i$ polyregular and $g_i$ quantifier-free, such that  for every input tree $t$, the tree $\restrict{f(t)} i$ is obtained by applying $g_i$ to the pair consisting of  $f_i(\restrictmore{ t}{i})$ and 
 $\restrict t i$. 

there exist functions 
\begin{align*}
f_0, f_{\half}, f_1, \ldots, f_{k - \half}, f_k : 
: \treesdown(\tau) \to \treesdown(\sigma)
\end{align*}
on partial trees, with the following properties: 
\begin{enumerate}
    \item for every $i \in \set{0,1,\ldots,k}$, there is a  quantifier-free interpretation 
    \begin{align*}
    f_i(t | i)  = f(t) | i
    \end{align*}
\end{enumerate}
following set of trees. Let $k$ be the maximal strength of $\tau$ and $\sigma$.  We say that $f$ is a \emph{good interpretation} if 

a set of sibling-ordered trees  set of trees $\trees \tau$ as follows. For $1$, the set of trees $\trees 1$ contains only one tree, 
For a datatype $\tau$, its \emph{tree semantics} is a set of trees that is defined as follows. The tree semantics of $1$ contains one tree 

==> fold.tex <==

\section{Fold}
\label{sec:introduction-to-fold}
Polyregular functions have many good closure properties.  For example, they  are closed under applying map:  if $f : \tau \to \sigma$ is polyregular, then the same is true for its lifting to  lists 
\begin{align*}
[A_1,\ldots,A_n] \in \tau^* \quad \mapsto \quad  [f(A_1),\ldots,f(A_n)] \in \sigma^*.
\end{align*}
Other closure properties of the polyregular functions include composition, or pairing.  The operation that is central to this paper is the \emph{fold} combinator,

\input{function-iteration}
which is defined as follows.
Consider a function 
\begin{align*}
\delta : \tau \times \sigma \to \tau,
\end{align*}
which should be thought of as the transition function of   some automaton, with state space $\tau$ and input alphabet $\sigma$. The state space input alphabet need not be finite, e.g.~the state space could be $1^*$, i.e.~the natural numbers. We will refer to functions of such type as \emph{automata}. The \emph{fold} of $\delta$ is defined to be the function 
\begin{align*}
\delta^* : \tau \times \sigma^* \to \tau,
\end{align*}
which is defined inductively on the second argument: 
\begin{align*}
\delta^*(\_,[]) & = \text{identity}\\
\delta^*(\_,[B_1,\ldots,B_n]) & = \delta(\_,B_1); \delta^*(\_,[B_2,\ldots,B_n]).
\end{align*}
In this paper, we are interested conditions on the transition function $\delta$ which ensure that its fold  is polyregular. 



\begin{theorem}\label{thm:fold-quantifier-free}
    Let $\tau$ and $\sigma$ be  classes of  structures, and let 
    \begin{align*}
    \delta : \sigma + \tau \times \sigma \to \tau
    \end{align*}
    be a quantifier free interpretation. Then its fold
    \begin{align*}
        \delta^* :  \tau \times \sigma^*  \to \tau
    \end{align*}
    is polyregular.
\end{theorem}
\begin{proof}
    In fact, we will prove that the fold of $\delta$ is a polyregular of dimension 1, in particular it is an \mso transduction. 

    The proof is based on transformations on quantifier-free types. The main ingredient of the proof will be Lemma~\ref{lem:quantifier-free-transformations}, which explains how the fold affects quantifier-free formulas. Suppose that we have an input to the fold which is of the form 
    \begin{align*}
    (A,[B_1,\ldots,B_n])
    \end{align*}
    together with some distinguished elements $c_1,\ldots,c_k$ in the input. Some of the distinguished elements may be from $A$, some may be from $[B_1,\ldots,B_n]$. 
    For a quantifier-free formula $\psi(x_1,\ldots,x_k)$ over the vocabulary of $\tau$, we will want to know if 
    \begin{align*}
        \delta^*(A,[B_1,\ldots,B_n]) \models \varphi(c_1,\ldots,c_k).
    \end{align*}
    Note that in order for the above hold, not only must the formula $\varphi$ be true, but also the elements $a_1,\ldots,a_n$ must be present in the structure, i.e.~they must not be deleted when applying the quantifier-free interpretations that define fold.  The main observation in the proof of the theorem is that this can be done in \mso. 

    \begin{lemma}\label{lem:quantifier-free-transformations}
        For every quantifier-free formula $\varphi(x_1,\ldots,x_k)$ over the vocabulary of $\tau$, there is an \mso formula $\psi(x_1,\ldots,x_k)$ such that 
        \[
        \begin{tikzcd}
            (A,[B_1,\ldots,B_n]) \models \psi(c_1,\ldots,c_k) 
            \ar[d,Leftrightarrow]\\
            \delta^*(A,[B_1,\ldots,B_n]) \models \varphi(c_1,\ldots,c_k).
        \end{tikzcd}
        \]
        holds  for every structure $(A,[B_1,\ldots,B_n]) \in \tau \times \sigma^*$ and distinguished elements  $c_1,\ldots,c_k$ in it.
    \end{lemma}
    \begin{proof}
        We begin by introducing some notation.  Consider a quantifier-free interpretation $f$, e.g.~$\delta(\_,B)$ for some fixed $B$. We will apply $f$ not just to structures, but also to structures with distinguished elements,  as explained below.
        If $A$ is an input structure, and $\bar a$ is a tuple of distinguished elements in it, then we write $f(A,\bar a)$ for the pair which consists of the structure $f(A)$ together with the same tuple of distinguished elements $\bar a$. The value $f(A, \bar a)$ is defined only if  all elements in the tuple $\bar a$ are indeed part of the universe of $f(A)$, i.e.~each element in the tuple satisfies the universe formula of the unique component in the interpretation. If some element in $\bar a$ is not part of the universe of $f(A)$, then $f(A, \bar a)$ is undefined. 
    
        If $A$ and $B$ are two structures over the same vocabularies, and $\bar a \in A^k$ and $\bar b \in B^k$ are two tuples of distinguished elements of equal length $k$, then we write 
        \begin{align*}
        A, \bar a \equiv B, \bar b
        \end{align*}
        if the same quantifier-free formulas are satisfied by both sides of the equivalence. An equivalence class of the above equivalence is called an \emph{quantifier-free type}. The following claim, which is an immediate corollary of the definitions and thus given without proof, says that quantifier-free equivalence, on structures with distinguished elements, is a congruence with respect to quantifier-free interpretations.
    
        \begin{claim}\label{claim:congruence}
            Let $f$ be a quantifier-free interpretation, and consider two inputs with distinguished elements which have the same quantifier-free type
            \begin{align*}
            (A,\bar a) \equiv (B, \bar b).
            \end{align*}
            Then after applying $f$, either both outputs  are undefined, or both outputs are defined and satisfy 
            \begin{align*}
                f(A,\bar a) \equiv f(B, \bar b).
            \end{align*}
        \end{claim}
        By the congruence property from the above claim, a quantifier-free interpretation can be lifted to a transformation on quantifier-free types. Importantly, there are finitely many quantifier-free types once the vocabulary and number of distinguished variables are fixed, and therefore the transformations on quantifier-free types will have domains and co-domains that are finite. 

        We now resume the proof of the lemma. We will prove the lemma in two steps. In the first step, we prove the special case where we assume that the distinguished elements $c_1,\ldots,c_k$ are from $A$, i.e.~they are from the initial state. In the second step, we prove the lemma in full generality. 

        \paragraph*{First step.} In this step we assume that the distinguished elements $c_1,\ldots,c_k$ are all from $A$. 
        To discuss quantifier-free types of structures with distinguished elements, we use the following notation:
    \begin{align*}
    \pointed k \tau \quad \eqdef \quad  \myunderbrace{\setbuild{(A,\bar a)}{$A \in \tau$ and $\bar a \in A^k$}}{structures from $\tau$ with $k$ distinguished elements}.
    \end{align*}
    The possible  quantifier-free types of such structures with distinguished elements will be denoted by $\typequot{(\pointed k \tau)}$. In terms of this notation, Claim~\ref{claim:congruence} applied to the quantifier-free interpretations of the form $\delta(\_,B)$ says that  for every $B \in \sigma$ there is a partial function 
    \begin{align*}
        F_B :   \typequot{(\pointed k \tau)}  \to 
        \typequot{(\pointed k \tau)} 
    \end{align*}
    such that for every $A \in \tau$ and distinguished elements $a_1,\ldots,a_k \in A$, the quantifier-free type of 
    \begin{align}\label{eq:output-quantifier-free-type}
    \delta(A,B), \bar a
    \end{align}
    is obtained by applying $F_B$ to the quantifier-free type of  $A, \bar a$. Furthermore, the output of the partial function is defined if and only if the quantifier-free type~\eqref{eq:output-quantifier-free-type}  is defined, i.e.~all of the elements from $\bar a$ are present in $\delta(A,B)$. Finally, the function $F_B$ depends only on the quantifier-free type of $B$ (without distinguished elements), which is the values of the predicates of $B$ that have arity zero. 

    By composing the functions $F_B$, we see that the quantifier-free type of 
    \begin{align*}
    \delta^*(A,[B_1,\ldots,B_n]), \bar a,
    \end{align*}
    which may be undefined, is obtained by taking the quantifier-free type of  $A, \bar a$, and applying to it the composition of the partial functions 
    \begin{align*}
    F_{B_1},\ldots, F_{B_n}.
    \end{align*}
    Therefore, in order to finish the proof of the lemma, it remains to show that a formula of \mso can compute the composition of these partial functions. This is done in the same way as computing the run of an automaton in \mso; here it is important that the set of possible partial functions of type 
\begin{align*}
    \typequot{(\pointed k \tau)}  \to 
    \typequot{(\pointed k \tau)} 
\end{align*}
is finite. This completes the proof of the first step. 

\paragraph*{Second step.} Consider now the general case of the lemma, where the elements $c_1,\ldots,c_k$ are not necessarily all from $A$.  The proof is by induction on $k$. Define the \emph{index} of an element of the input structure to be $0$ if the element comes from $A$, otherwise it is $i \in \set{1,\ldots,n}$ if the element comes from $B_i$. Consider the maximal index $i \in \set{0,\ldots,n}$ that is used by the distinguished elements, and let $\bar c$ be the tuple $\bar a$ restricted to elements of index $<i$. This is a shorter tuple, and therefore we can use the  induction assumption, to see that   \mso can determine the quantifier-free type of 
    \begin{align*}
    \delta^*(A,[B_1,\ldots,B_{i-1}]), \bar c.
    \end{align*}
    By applying one step of the transition function, we can use \mso to find the quantifier-free type of 
    \begin{align*}
    \delta^*(A,[B_1,\ldots,B_i]), \bar a.
    \end{align*}
    Finally, if we think of the above as an initial state with distinguished elements, and we think of the input string as being $[B_{i+1},\ldots,B_n]$, then  we can use the already proved first step  to compute in \mso the quantifer-free type of 
    \begin{align*}
        \delta^*(A,[B_1,\ldots,B_n]), \bar a.
        \end{align*}
    as required by the lemma.
\end{proof}

    Having proved the lemma, we can complete the proof of the theorem. By applying the lemma to the quantifier-free formula
    \begin{align*}
    \varphi(x_1) = \text{true},
    \end{align*}
    we see that there is an \mso formula which tells us which elements of the input structure are part of the output structure. The relations on the output structure are defined in a similar way, by viewing each relation symbol as a quantifier-free formula.
\end{proof}



==> function-iteration.tex <==
\subsection{Function iteration}



As the two above examples show, we have to be careful when applying iteration fold. Clearly we have to avoid duplication (Example~\ref{ex:fold-duplication}). It is less clear what the problem with Example~\ref{ex:fold-tail} is; our perspective is that the problem is that the iterated function  uses quantifiers.  
For this reason, we will care about \emph{quantifier-free interpretations}

\begin{definition}
    A \emph{quantifier-free interpretation} is the special case of \mso interpretations where all formulas are required to be quantifier free, there is a unique component of dimension one, and  no component of dimension bigger than one.
\end{definition}
the dimension is $k=1$. For quantifier-free interpretations, fold is polyregular. 


\begin{lemma}
    If a function 
    \begin{align*}
    f : \tau \to \tau
    \end{align*}
    is a quantifier-free interpretation, then its iteration
    \begin{align*}
        f^\# :  \tau \times 1^* \to \tau
        \end{align*}
    is an \mso interpretation of dimension 1.
\end{lemma}
\begin{proof}
    Let $M$ be the set of quantifier-free interpretations of type $\tau \to \tau$. This is a monoid, with the monoid operation being composition, since the quantifier-free interpretations are closed under composition. Crucially, this monoid is finite, since there are finitely many quantifier-free formulas that can be written to define the universe and the relations.  The function of type $1^* \to M$ defined by 
    \begin{align*}
    1^n \quad \mapsto \quad f^n
    \end{align*}
    is a monoid homomorphism into a finite monoid, and therefore it is definable in \mso  in the sense that for every possible value $g \in M$ there is an \mso formula defining defining 
    \begin{align*}
    \setbuild { 1^n }{ $f^n = g$}.
    \end{align*}
    This completes the proof of the lemma: to compute the iteration $f^\#(A,1^n)$, we first use an \mso formula evaluated in $1^n$ to compute the function $f^n$, and then we apply it to $A$. 
\end{proof}




\newcommand{\submodel}[2]{#1|\text{(#2)}}

We begin by introducing some notation. Consider some input to the fold function 
\begin{align*}
(Q_0, [A_1,\ldots,A_n])\in \tau \times \sigma^*.
\end{align*}
In the proof below, when speaking of the input, we mean the above. We will use automata terminology in the proof, i.e.~we will refer to $Q_0$ as the \emph{initial state}, and we will use the name \emph{input letters} for the structures $A_1,\ldots,A_n$. 
For $i \in \set{1,\ldots,n}$, define $Q_i \in \tau$ to be the state of the automaton after reading the first $i$ letters, i.e. 
\begin{align*}
Q_{i} = \delta(Q_{i-1},A_{i}).
\end{align*}
The output of the fold function is the last state  $Q_n$, but in order to compute it, we will actually compute all states $Q_1,\ldots,Q_n$. 

Define a \emph{state element} to be an element of the universe in one of the state structures $Q_0,\ldots,Q_n$. We will also be interested in a \emph{parent function}, which is a partial function that maps  state elements from $Q_{i}$ to possibly undefined state elements from $Q_{i-1}$, as described below.  When a state  $Q_i$ is produced by applying the transition function to the pair $(Q_{i-1},A_i)$, we can classify the elements in the universe of  $Q_i$ into two kinds:
\begin{itemize}
\item equi-grade elements that belong to $Q_{i-1}$; and
\item the remaining elements, i.e.~down-graded elements, or equi-grade elements that belong to $A_i$.
\end{itemize}
For elements of the first kind, the \emph{parent} is defined to be the corresponding element in $Q_{i-1}$, and for elements of the second kind, the parent is undefined. 
% Let us write $Q^\ell_i$ for the elements of $Q_i$ that have grade $\ge \ell$ and origin exactly $i$, in other words they have grade $\ge \ell$ and kind (a). 
Define the \emph{run structure} to be the structure 
\begin{align*}
R = [Q_0,A_1,Q_1,\ldots, A_n,Q_n] \in (\tau + \sigma)^*
\end{align*}
together with the parent function. To prove the theorem, we will show  that the run structure can be computed by a graded polyregular function, in a way such that all state elements are down-graded. We will do this grade by grade, in the following sense. For a grade $\ell$, define \emph{grade $\ell$ run structure} $R_\ell$ to be the result of removing from the run structure the elements of $Q_1,\ldots,Q_n$ that have grade strictly smaller than  $\ell$. (All elements of $Q_0$ and $A_1,\ldots,A_n$ are kept, regardless of their grades.)  By induction on $\ell$, we will show that the grade $\ell$ run structure can be computed by a graded polyregular function. The induction is in the opposite order: the induction basis is when $\ell$ is one plus the maximal grade that appears in the input, and it proceeds down to $\ell=0$, in which case the run structure is obtained. In the induction basis there is nothing to do, since in this case the grade $\ell$ run structure contains no elements from $Q_1,\ldots,Q_n$. 

The rest of the proof is devoted to the induction step. Suppose that we already have the grade $\ell+1$ run structure, and we want to produce the grade $\ell$ run structure. 



For an element of $Q_i$ or $A_i$, the number $i$ is called its \emph{index}. 
For a state element, define its \emph{progenitor} to be the unique ancestor (i.e.~transitive reflexive closure of the parent relation) that has no parent. Since the parent function is injective (i.e.~there cannot be two state elements with the same parent), it follows that for every state element is represented uniquely by  is represent uniquely by its progenitor and its index. Therefore, we write $a@i$ for the at most one state element that has progenitor $a$ and index $i$. The element $a@i$ is undefined if there is no element in $Q_i$ that has progenitor $a$. We will also want to represent the index as an element of the run structure, and not as a number: to do this, we define the \emph{representation} of $i$ to be the unique king element of $A_i$. We overload the notation as follows: if $b$ is the representation of an index $i$, then we write $a@b$ as a synonym for $a@i$, otherwise $a@b$ is undefined. 

 We want this representation to be a pair of elements in the run structure, and therefore the index will be represented using the unique king element in the structure $A_i$. Summing up, the \emph{progenitor representation} of a state element from $Q_i$ is the pair (the progenitor, the king element of $A_i$). We write $a@b$ for the element which has progenitor representation $(a,b)$, this is element might not be defined, but if it is defined then it is unique. 

Consider a pair of elements $(a,b)$ in the run structure such that: (i) $a$ is a state element without a parent; and (ii)  $b$ is the king element of some $Q_i$ which contains an element with progenitor $a$. We  write $a@b$ for the unique element in $Q_i$ that has progenitor $a$. Otherwise $a@b$ is undefined, i.e.~it is undefined if either $a$ is not a state element without a parent, or 


the progenitor of $c$ and the 

For $i \in \set{1,\ldots,n}$, we define the \emph{representation of $i$} to be the element of the run structure which is the chosen element of $A_i$. Elements of  $Q_1,\ldots,Q_n$ in the run structure are called \emph{state elements}, the remaining elements of the run structure are called \emph{input elements}. The following notation will be key: the representation of state element $c$ in the run structure is the pair $(a,b)$ such that $a$ is a state element with no parent, $b$ is the representation of an index 

 






Let us define $Q^\ell_i$ to be the result of restricting the structure $Q_i$ to elements which either: (a) have grade $>\ell$; or (b) have grade exactly $\ell$ and no parent. The following claim shows that these structures can be computed, using \mso interpretations, based on the available information:



\begin{claim}
    There is an \mso formula $\varphi(x,y)$ such that for every input to the fold,
    \begin{align*}
    R_{\ell + 1} \models \varphi(a,b) \qquad \text{iff} \qquad \text{$a@b$ is defined}.
    \end{align*}
    \end{claim}


\begin{claim} Let $\psi(x_1,\ldots,x_k)$ be an \mso formula over the vocabulary of $\tau$.  
    There is an \mso formula $\varphi(x_1,\ldots,x_k,y)$ such that for every input to the fold,
    \begin{align*}
    R_{\ell + 1} \models \varphi(a_1,\ldots,a_k,b)
    \end{align*}
    holds if and only if: $a_1@b, \ldots, a_k@b$ are all defined and 
    satisfy 
    \begin{align*}
    Q_b \models \varphi(a_1@b,\ldots,a_k@b)
    \end{align*}
\end{claim}


\begin{claim}\label{claim:equi-grade}
    There is an \mso interpretation
    \begin{align*}
    \gamma : \tau \times \sigma \to \tau,
    \end{align*}
     which depends only on $\ell$ and not the input, such that  
    \begin{align*}
    Q^\ell_i = \gamma(\submodel{(Q_{j-1},A_j)}{grade $> \ell$})
    \end{align*}
    holds for every input and every $i \in \set{1,\ldots,n}$. 
\end{claim}

\begin{claim}\label{claim:down-grade}
    For every $i \in \set{1,\ldots,n}$ there is a quantifier-free interpretation 
    \begin{align*}
    f_i : \tau \to \tau,
    \end{align*}
    which depends only on the quantifier-free theory of $A_i$, such that 
    \begin{align*}
    \submodel{Q_{i}} {origin $<i$} = f_i(\submodel{Q_{i-1}} {origin $<i$})
    \end{align*}
\end{claim}


By Claims~\ref{claim:equi-grade} and~\ref{claim:down-grade},  for every $j \le i \in \set{1,\ldots,n}$, we have
\begin{align*}
\submodel{Q_i}{origin $j$ and grade $\ge \ell$} =  \myunderbrace{f_{i} \circ f_{i-1} \circ \cdots \circ f_{j+1}}{call this $f_{ij}$}(Q^\ell_j).
\end{align*}
The function $f_{ij}$ belongs to the finite monoid of quantifier-free interpretations of type $\tau \to \tau$, and therefore similarly to Lemma~\ref{lem:}, it can be computed in \mso based on the indices $i$ and $j$ as well as the input $[A_1,\ldots,A_n]$. 
By induction assumption, the structure 
\begin{align*}
[Q_1^\ell, \ldots, Q_n^\ell]
\end{align*}
can be computed by an \mso interpretation.


==> knowledge.tex <==
\knowledgeconfigure{protect quotation={tikzcd}}

\knowledge{notion,color=black}
 | structure

==> new-proof.tex <==
\newcommand{\elind}[1]{\underline{#1}}
\newcommand{\sucat}[2]{#1 @ \elind{#2}}

\begin{lemma}
    Let $\sigma$ and $\tau$ be graded datatypes. 
    If 
    \begin{align*}
        \delta : \tau \times \sigma  \to \tau
    \end{align*}
    is graded polyregular, then the same is true for its fold
    \begin{align*}
        \delta^* :  \upgrade{(\tau \times \sigma^*)} \to \tau
    \end{align*}
\end{lemma}
\begin{proof}
    In the output of the transition function 
    \begin{align*}
    \delta(A,B)
    \end{align*}
    we will distinguish two types of elements: the downgraded elements, and the equigrade elements. For each equigrade output element there is a corresponding element of the same grade in the input structure, which is called its \emph{parent}. Parents are undefined for downgraded elements.  We extend these notions to the fold
    \begin{align*}
    \delta^*(A,[B_1,\ldots,B_n])
    \end{align*}
    as follows: an output element is called downgraded if it has a defined parent  in the last application of $\delta$, and that parent  is either in $B_n$ or it is an equigrade element of 
    \begin{align*}
    \delta^*(A,[B_1,\ldots,B_{n-1}]).
    \end{align*}

    Like for any graded polyregular function, if we restrict to output of the transition function to the  equigrade elements, then it becomes quantifier-free, i.e.~the function 
    \begin{align*}
    \myunderbrace{(A,B) \quad \mapsto \quad \delta(A,B)|\text{equigrade}}{call this function $\delta_=$}
    \end{align*}
    is a quantifier-free interpretation. Therefore, by applying  Lemma~\ref{lem:quantifier-free-transformations} to $\delta_=$ we see that  conclude that for every quantifier-free formula $\varphi(x_1,\ldots,x_k)$ over the vocabulary of $\tau$, there is a quantifier-free formula $\psi(x_1,\ldots,x_k)$ such that 
    \[
        \begin{tikzcd}
            (A,[B_1,\ldots,B_n]) \models \psi(c_1,\ldots,c_k) 
            \ar[d,Leftrightarrow]\\
            \delta^*_=(A,[B_1,\ldots,B_n]) \models \varphi(c_1,\ldots,c_k).
        \end{tikzcd}
        \]
        holds  for every structure $(A,[B_1,\ldots,B_n]) \in \tau \times \sigma^*$ and distinguished elements  $c_1,\ldots,c_k$ in it.

    We begin by explaining some notation, which will be used in the proof. 
    Consider an input to the fold, which is of the form 
    \begin{align*}
     \upgrade{(A,[B_1,\ldots,B_{n}])} \in \upgrade{(\tau \times \sigma^*)}.
    \end{align*}
    Apart from the initial state $A$, we will be interested in all other states in the run of the automaton, using the following notation: 
\begin{align*}
A_1 = A \qquad A_{i+1} = \delta(A_i,B_i).
\end{align*}
The output of the fold, and the value that we ultimately want to compute, is $A_{n+1}$. By definition of graded polyregular functions, the value $A_{i+1}$ is computed in two stages: an expansion $\delta_1$, followed by a quantifier-free interpretation $\delta_2$, as in the following diagram: 
\[
\begin{tikzcd}
(A_i,B_i) 
\ar[r,mapsto,"\delta_{\downarrow}"]
&
\delta_{\downarrow}(A_i,B_i)
\ar[r,mapsto,"\delta_{qf}"]
&
B_{i+1}
\end{tikzcd}
\]
The expansion adds elements and keeps the input structure intact, while the quantifier-free interpretation removes elements. Therefore, there are two natural embeddings, which are described below:
\[
\begin{tikzcd}
(A_i,B_i) 
\ar[r,hookrightarrow,"\alpha_i"]
&
\delta_{\downarrow}(A_i,B_i)
\ar[r,hookleftarrow,"\beta_i"]
&
B_{i+1}
\end{tikzcd}
\]
Define $C$ to be the structure 
\begin{align*}
[\Delta(A_1,B_1), \ldots, \Delta(A_n,B_n) ].
\end{align*}
We will prove that $C$ can be computed from the input structure by a graded polyregular function; this will complete the lemma since the output of the fold is obtained from $C$ by applying a quantifier-free interpretation to the last element of the list. 

The general idea is to define the structure $C$ grade by grade, starting with the highest grade and proceeding down to grade zero. More precisely, for $\ell \in \set{0,1,\ldots}$, define $C|\ell$ to be the structure obtained from $C$ by keeping only the elements of grade at least $\ell$. 
An element of $C$ is called \emph{downgraded} if for some $i \in \set{1,\ldots,n}$ it belongs to $\Delta(A_n,B_n)$ but it does not belong to $(A_n,B_n)$. 

together with two  binary relations $\alpha$ and $\beta$ that represent the union of, respectively, the embeddings $\alpha_i$ and $\beta_i$. An element of $C$ is called \emph{downgraded} if for some $i \in \set{1,\ldots,n}$ it belongs to $\delta_1(A_i,B_i)$ but it does not belong to $(A_i,B_i)$. 

    For $i \in \set{0,\ldots,n}$ define $B_{i+1} \in \tau$ to be the result of applying the fold to 
    \begin{align*}
    \upgrade{(B,[R_1,\ldots,R_{i}])}.
    \end{align*}


    
    By definition of fold, $B_1 = B$ and 
    \begin{align*}
    B_{i+1} = \delta(B_i,R_i) \qquad \text{for $i \in \set{1,\ldots,n}$.}
    \end{align*}
    Ultimately, we will be interested in the last element $B_{n+1}$, but the preceding list elements will also need to be computed.  Again, if $A$ is clear from the context we will use the variables  $B_1,\ldots,B_{n+1}$ in the above sense. 

    \paragraph*{Some terminology.}
    Elements of the structures $Q_1,\ldots,Q_n$ will be called \emph{letter elements}, and elements of the structures  $B_1,\ldots,B_{n+1}$ will be called \emph{state elements}. The state elements will be further classified into two groups: the \emph{initial state elements}  are from $B_1$, and the \emph{non-initial state elements} are from $B_2,\ldots,B_n$. The difficult part will be computing the non-initial state elements and the relations on them.  Consider a state  $Q_i$ with  $i \in \set{1,\ldots,n}$. This state is obtained by taking  $(Q_{i-1},A_i)$, applying the down-grading part of $\delta$, and then applying the quantifier-free part of $\delta$. This leads to two origin maps: the origin map of the down-grading part 
    \[
    \begin{tikzcd}
    P_i 
    \ar[r]
    & 
    \displaystyle{
    \coprod_{\alpha} (Q_{i-1},A_i)^{\text{dimension of $\alpha$}}}
    \end{tikzcd}
    \]
    and the origin map of the quantifier-free part, which is a grade-preserving  inclusion
    \[
    \begin{tikzcd}
    Q_i 
    \ar[r,hookrightarrow]
    &
    P_i.
    \end{tikzcd}
    \]
    Furthermore, the down-grading part must keep its input intact, and therefore there is also a grade-preserving inclusion 
    \[
    \begin{tikzcd}
    (Q_{i-1},A_i)
    \ar[r,hookrightarrow]
    &
    P_i.
    \end{tikzcd}
    \]
    
    
every element  $q \in Q_i$ is of one of two kinds: 
    \begin{itemize}
    \item it is equal to some element of $(Q_{i-1},A_i)$ with the same grade; or 
    \item 
    \end{itemize}
    
    and consider an element $q$ of a state structure $Q_i$ Every element of a state structure $q \in Q_i$, with $i \in \set{1,\ldots,n}$ is of the form 
    \begin{align}\label{eq:origins}
    b = \myunderbrace{q(d_1,\ldots,d_k)}{this is called the \emph{origin} of $b$}
    \end{align}
    where $q$ is some component of the transition function, $k$ is the dimension of $q$, and $d_1,\ldots,d_k$ are elements of $(B_i,A_i)$.  We say that $b$ is \emph{down-graded}  if all elements in its origin have grade strictly bigger than $b$, otherwise we say that $b$ is \emph{equi-graded}. 

    \paragraph*{The induction.} To prove the lemma,  we will study  a structure, called the run structure, which consists of the structure 
\begin{align*}
(Q_0,[(A_1,Q_1),\ldots,(A_n,Q_n)])
\end{align*}
    together with the following auxiliary information: for every component $\alpha$ of the transition function, of dimension $k$, the run structure  is equipped with a relation of arity $k+1$ that describes the relation~\eqref{eq:origins}. 
    

    We write $R$ for the run structure. It depends on the input, so we will  write $R(Q,A)$ if the input  is not implicit from the context. 
    To prove the lemma, we will show that the run structure  can be produced from the input using a graded polyregular function. The proof is by induction on grades in the following sense: the run structure  will be produced grade by grade, starting with the elements of the highest grade and progressing down to the elements with the lowest grade. For $\ell \in \set{0,1,\ldots}$,  define the run structure of grade $\ell$, denoted by $R_\ell$,  to be the structure which is obtained from the run structure by removing elements of $Q_1,\ldots,Q_n$ that have  grade $< \ell$.  When $\ell$ exceeds the maximal grade that can appear in the output of the fold, then the run structure of grade $\ell$ is the same as the input, and  therefore it can be produced from the input using a graded polyregular function. The rest of the proof is devoted to showing that for every  $\ell$, the function 
    $R_{\ell+1} \mapsto  R_\ell$
    is graded polyregular.   Since graded polyregular functions are closed under composition,   it will follow that  the $R_0 = R$ can be produced from the input using a  graded polyregular polyregular function.

    % \newcommand{\chalf}{R_{\ell+1/2}}
    The rest of this proof is devoted to defining $R_\ell$ in terms of  $R_{\ell+1}$. The difficult part will be understanding the elements of level exactly $\ell$ that are created somewhere in the run, and then passed transferred to later states without decreasing their grades. To describe these elements, we use the following parent relation: we say that $a \in Q_{i-1}$ is the \emph{parent} of $b \in Q_i$ if both $a$ and $b$ have grade $\ell$, and  $b$ is the origin of  $a$. The parent relation is only used to relate elements of grade $\ell$  belonging to consecutive states; in particular if an element of $Q_i$  has origin in $A_i$, then it has no parent. The \emph{child} relation is defined to be the converse of the parent relation, and the \emph{ancestor} relation is defined to be the reflexive transitive closure of the parent relation. Every element has at most one parent and, because  a graded polyregular function had at most one equi-grade component in each grade, every  element has at most one child. 
    
    
    Define $\chalf$ to be the structure obtained from $R_\ell$ by removing elements that have a defined parent. 
    
    \begin{claim}
         $R_{\ell+1} \mapsto \chalf$ is graded polyregular. 
    \end{claim}
    \begin{proof}
        To the input structure we need to add the iterated output elements that are  down-graded elements and have grade exactly  $\ell$. These are represented using their origins (which are present already in $R_{\ell+1}$) and all  relations in the output structure can be easily extended, using \mso, to account for the new elements by using the state update function.
    \end{proof}
    
    We now proceed to the core of the proof, which is computing the grade $\ell$ run structure  $R_\ell$ by applying a graded polyregular function to $\chalf$.  As in the above claim, we only need to define the new elements, i.e.~elements that have a defined parent, and the relations of the run structure structure on tuples that involve at least one new element. These new elements can be described as follows. Define an element of index $i$ to be an element of $Q_i$ or $A_i$. 
    Every element has a unique ancestor that has no parents; this ancestor is called its \emph{progenitor}. An element is uniquely specified by its progenitor and index; we write $a@i$ for the at most one element that has progenitor $a$ and index $i$. The pair $(a,i)$ is called the \emph{progenitor representation} of the element $a@i$. The following claim shows that whether or not the progenitor-representation is defined can be checked by an \mso formula. 

    \begin{claim}\label{claim:progenitor-defined}
         Let us write  $\underline b$ to denote the index of an element $b$. 
        There is an \mso formula $\varphi$ such that 
        \begin{align*}
        \chalf \models \varphi(a,b) \qquad \text{iff} \qquad a@\underline b\text{ is defined}.
        \end{align*}
    \end{claim}
    \begin{proof}
        Let $i$ be the index of $b$ and let $j$ be the index of $a$. In terms of this notation, $a@\underline b$ is defined if and only if  $a$ has a descendant that has index $j$. If $j < i$ then this descendant does not exist, and if $j = i$ then this descendant vacuously exists, since it is $a$ itself. The interesting case is deciding if such a descendant exists when $j > i$. This means that we need to check if $a$ has a child, and that child has a child, and so on until index $i$ is reached. To check this in \mso, we will use the same technique of composing quantifier-free interpretations that was used in the proof of Lemma~\ref{lem:quantifier-free-transformations}.
        
          
        Because the transition function is graded polyregular, for every $m \in \set{j+1,\ldots,i}$ there is a quantifier-free interpretation $f_i : \tau \to \tau$ such that
        $f_i(Q_{i-1})$  is the  structure $Q_i$ restricted to elements with defined parent. Furthermore, this interpretations depends only on $A_i$, and more specifically on its quantifier-free type. If we compose the  interpretations 
        \begin{align*}
        \myunderbrace{f_{j+1}; f_{j+2}; \cdots; f_i}{let $f$ be this composition}
        \end{align*}
        and apply them to $Q_j$, then we get the structure $Q_i$ restricted to elements whose progenitor has index $\le j$. In particular, $a@j$ is defined if and only if $a$ belongs to $Q_j$ and  satisfies the universe formula of $f$. This can be checked in \mso, since $f$ can be computed in \mso based on $a$ and $b$ by using multiplication in the finite monoid of quantifier-free interpretations of type $\tau \to \tau$. 
    \end{proof}

    We will compute $R_\ell$ from $\chalf$, by defining the new elements using a component of dimension two which refers to the progenitor representation. The key is going to be Claim~\ref{claim:relations-on-progenitor-representation}, which shows that the relations in the structure $\chalf$ can also be defined in \mso, using the progenitor representation of elements. Before we prove the claim, however, we need a preliminary result, Claim~\ref{claim:parent-theory} below, which explains how quantifier-free theories of elements can be computed based on quantifier-free theories of their parents. 

     \begin{claim}\label{claim:parent-theory}
        There is a quantifier rank $r \in \set{0,1,\ldots}$ with the following property. Consider an input structure, and  elements 
        \begin{align*}
        \myunderbrace{a_1,\ldots,a_k}{$\bar a$},\myunderbrace{b_1,\ldots,b_\ell}{$\bar b$} \in Q_i
        \end{align*}
        such that all elements in $\bar a$ have defined parents, call them 
        \begin{align*}
            \myunderbrace{c_1,\ldots,c_k}{$\bar c$} \in Q_{i-1},
        \end{align*}
        and all elements in $\bar b$ have undefined parents. Then 
        \begin{align*}
        \text{quantifier-free type of }Q_i, \bar a, \bar b
        \end{align*}
        is uniquely determined by the following  types:
        \begin{align*}
        \text{quantifier-free type of }A_i\\
        \text{quantifier-free type of }Q_{i-1}, \bar c\\
        \text{rank $r$ \mso type of }\chalf, \bar b.
        \end{align*}
    \end{claim}
    \begin{proof}
        Using the definition of graded polyregular functions.
    \end{proof}


    Using the above claim, we can show how the structure of $R_\ell$ can be defined in \mso using the progenitor information.

    \begin{claim}\label{claim:relations-on-progenitor-representation}
        Let $\psi(x_1,\ldots,x_k)$ be a quantifier-free formula over the vocabulary of the run structure.  There is an \mso formula $\varphi$ over the same vocabulary with $2k$ free variables  such that 
        \begin{align*}
        \chalf \models \varphi(a_1,b_1,a_2,b_2,\cdots,a_k,b_k) 
        \end{align*}
        holds if and only if
        all pairs $(a_1,b_1), \ldots, (a_k,b_k)$ are progenitor representations, say of elements $c_1,\ldots,c_k$, and the 
        \begin{align*}
        R_\ell \models \psi(c_1,\ldots,c_k).
        \end{align*}
        \end{claim}
        \begin{proof}
            It is enough to prove the claim when the quantifier-free formula is an atomic relation of the structure $\chalf$; since other quantifier-free formulas can be obtained by applying Boolean combinations. Among the atomic relations, the only interesting case is atomic relations from the vocabulary of $\tau$. Suppose then, for the rest of this proof, that $\varphi$ is an atomic relation from the vocabulary of the class $\tau$. In this case, all of the elements $c_1,\ldots,c_k$ must belong to the same state structure, which means that all $b_1,\ldots,b_k$ are equal, and are the leader of some $i \in \set{1,\ldots,k}$.  Let $j \le i$ be the maximal index of the elements  
            The only interesting case is when all of the elements $c_1,\ldots,c_k$ are defined, and they belong to the same state $Q_i$. 

            Let $j$ be the maximal index among $a_1,\ldots,a_k$. For  $m \in \set{j,\ldots,i}$ define $T_m$ to be the quantifier-free type of $Q_m$ with distinguished elements
            \begin{align*}
            a_1@m, \ldots, a_k@m.
            \end{align*}
            By choice of $m$, all of these distinguished elements are defined. We will proceed in two steps: (1) first we show that $T_j$ can be computed in \mso; and then we show that (2) $T_i$ can be computed from $T_j$. 

            \begin{enumerate}
                \item \emph{Computing $T_j$.} By maximality of $j$, we know that at least one of the elements $a_1@j, \ldots, a_k@j$ has undefined parent.  Without loss of generality, assume that the parent is defined for the first  $p \in \set{1,\ldots,k-1}$ elements, and it is undefined for the remaining $k-p$ elements. By Claim~\ref{claim:parent-theory}, the quantifier-free type  $T_j$ is uniquely determined by the following three pieces of information:
                \begin{enumerate}
                \item the quantifier-free type of $A_j$ without distinguished elements;
                \item the quantifier-free type of $Q_{j-1}$ with distinguished elements  
                \begin{align*}
                    a_{1}@(j-1),\ldots,a_{p}@(j-1),
                \end{align*}
                \item the rank $r$ (as in the Claim) \mso type of $\chalf$ with distinguished elements
                \begin{align*}
                a_{p+1}@j, \ldots, a_k@j.
                \end{align*}
                \end{enumerate}
                The first and third piece of information are clearly definable  in \mso in the structure $\chalf$. For the second piece of information, it is definable in \mso thanks to the induction assumption on $k$. 
                \item \emph{Computing $T_i$.} By Claim~\ref{claim:parent-theory}, for every  $m \in \set{j+1,\ldots,i}$ the type $T_{m}$ depends only on the quantifier-free type of $A_m$ and the type $T_{m-1}$.  This means that there is some transformation $f_m$ on quantifier-free types such that 
                 \begin{align*}
                    T_m = f_m(T_{m-1}),
                \end{align*}
                and furthermore this transformation  depends on the quantifier-free type of $A_m$. 
                The quantifier-free type $T_i$ can be obtained by composing all of these functions, and applying them to $T_j$, as follows:
                \begin{align*}
                T_{j} \stackrel{f_{j+1}} \mapsto T_{j+1} \stackrel{f_{j+2}}  \mapsto T_{j+2} \stackrel{f_{j+3}}  \mapsto \cdots  \stackrel{f_{i}}  \mapsto T_i.
                \end{align*}
                Since all of the transformation belong to a finite monoid of constant size, their composition can be computed in \mso, and thus also $T_i$ can be computed, assuming that $T_j$ is already known.  
            \end{enumerate}
        \end{proof}

        The above claim gives us a representation of the new elements in $R_\ell$; each such element can be represented as $a@\underline b$, for some two elements $a,b \in \chalf$. Since there can be several choices for $b$ with the same index, thus leading to non-unique representations, we will require 
    that $b$ is a \emph{leader}, namely it is the unique leader element in $A_i$.  The important property of the leaders is that this is an \mso definable subset of  $\chalf$, and there is exactly one leader for every index.  Using the leaders, we define the \emph{progenitor representation} of an element in $c \in R_\ell$ as follows: this is the pair which consists of the progenitor of $c$ and the  leader of the index of $c$. In other words, this is the unique pair $(a,b)$ such that 
    \begin{align*}
    a@b = c \quad \text{and $b$ is a leader}.
    \end{align*}
    Every element of $R_\ell$ has a unique progenitor representation, the progenitor representation uses elements of $\chalf$, and  the set of pairs which are progenitor representations is definable in \mso. To produce $R_\ell$ from $\chalf$ using a graded polyregular function, the elements that are already in $\chalf$ will be copied using equi-grade components, while the new elements will be created using a down-graded component of dimension two, using the progenitor representation. 

    To complete the proof of the lemma, we need to show that the relations on the structure $R_\ell$ can be defined in \mso, in terms of the progenitor representation in the structure $\chalf$. This is stated in the following 

    
    \begin{proof}


    $(a,b)$ such that $c = a@\underline b$ and $b$ is a leader. 
    The new elements of $R_\ell$ are in bijective correspondence with the set set of pairs
    \begin{align*}
    \setbuild{(a,b)}{$b$ is a leader and $a@\underline b$ is defined},
    \end{align*}
    which is \mso definable. 
    . 
    Thanks to the above claim, the new elements in $R_\ell$ can be represented by pairs of elements in $\chalf$ in an \mso definable way. To make the representation unique, i.e.~so that every new element is represented by exactly one pair $(a,b)$, we can require $b$ to be some designated and \mso definable element of index $i$. 



     

    

        Thanks to the above claim, we can have access to the new elements in $R_\ell$, by representing them as pairs $c@\elind a$. This representation is interesting mainly for the  new elements of $R_\ell$, but it also applies to the remaining elements, since every element $c$ that was already in $ \chalf$ is equal to $c@\elind c$. In the following claim, we show that the relations in the structure $R_\ell$ can be defined in \mso in terms of $\chalf$, using the representation $c@a$.   

    
        To check if the tuple is entirely defined, we use Claim~\ref{claim:at-defined}. It remains to check if the relation is satisfied. The easy cases are when $R$ is one of the relations in the input structure $A$, the order on list elements in the output list $[B_1,\ldots,B_n]$, one of the origin relations, or the index relation.
        
        
        Suppose that we are given elements $c_1,\ldots,c_k \in \chalf$ and an index $i \in \set{1,\ldots,n}$,  and we want to  determine the quantifier-free type of 
        \begin{align*}
        Q_i, \myunderbrace{c_1@i,  \ldots, c_k@i}{distinguished elements in $Q_i$}.
        \end{align*}
        This type will be undefined if at least one of the elements $c_1@i, \ldots, c_k@i$ is undefined or does not belong to $Q_i$. By .., we know that for every $j \in \set{0,\ldots,i}$, the structure  \begin{align*}
            Q_i | \text{(progenitor has index $\le j$)}
            \end{align*} 
            is obtained from 
            \begin{align*}
            Q_j | \text{(progenitor has index $\le j$)}
            \end{align*}
            by applying some quantifier-free interpretation $f$, which can be computed using \mso based on the indices $i$ and $j$ and the input structure. Choose $j$ to be the minimal index in $\set{0,\ldots,i}$ such that  all of the elements  
        \begin{align*}
        c_1@j,\ldots,c_k@j 
        \end{align*}
        are defined, and are state elements, which means that they belong to $Q_j$. By .., the
       Therefore, since $f$ can be computed in \mso, in order to know that quantifier-free type of 
        \begin{align*}
        Q_i, \myunderbrace{c_1@i,  \ldots, c_k@i}{distinguished elements in $Q_i$}.
        \end{align*}
        it is enough to compute the quanitifier-free type of 
        \begin{align*}
            Q_j, \myunderbrace{c_1@j,  \ldots, c_k@j}{distinguished elements in $Q_i$}.
            \end{align*} 
        By minimality of $j$, some of the elements $c_1@j,\ldots,c_k@j$ have undefined parents, . Consider the origins 
        \begin{align*}
        c_1@j = \alpha_1(\bar a_k), \ldots, c_k@j = \alpha_k(\bar a_k)
        \end{align*}
        such that $\bar a_1,\ldots, \bar a_k$ are tuples of elements in $(Q_{j-1},A_j)$. Because the state update function is graded polyregular, we know that the quantifier-free theory of .. depends only on:
        \begin{itemize}
        \item the quantifier-free theory of 
        \begin{align*}
        (Q_{j-1},A_j), \bar a_1,\ldots, \bar a_k; 
        \end{align*}
        \item  the \mso theory of quantifier rank $r$ of 
        \begin{align*}
        ((Q_{j-1},A_j), \bar a_1,\ldots, \bar a_k) | \text{level $> \ell$}
        \end{align*}
        \end{itemize}
        
        $R$ is one of the relations in the vocabulary of $\tau$.  In this case, all of the elements $R_1@a_1,\ldots,R_k@a_k$ must have the same index, and therefore this index can be represented by a single element  $a$. Also, the index must be at least $2$, since all output elements of index 1 are already present in $\chalf$.
        
        
        % Summing up, to prove the claim it remains to show that for every relation name $R$ in the vocabulary of $\tau$, there is a formula $\varphi$ of \mso such that 
        % \begin{align*}
        % \chalf \models C(R_1,\ldots,R_k,a)
        % \end{align*}
        
        The formula defining this case will be defined by induction on  the following induction parameter. Define the \emph{grade profile} for a tuple $\bar c$   to be the following information: how many coordinates in the tuple have grade $\ell$, how many coordinates have grade $\ell+1$, and so on. Grade profiles are ordered lexicographically, which means that the grade profile decreases if one coordinate in the tuple is replaced by (possibly many) elements that have a strictly higher grade. By induction on grade profiles, we will show that for every grade profile $\pi$ and every relation name $R$ in the vocabulary of $\tau$,  there is an \mso formula $\varphi$ such that 
            such that 
        \begin{align*}
            \chalf \models \varphi(R_1,\ldots,R_k,a)
            \end{align*}
            holds if and only if $a$ has index at least two, the entire tuple 
            \begin{align*}
                \bar c @ \elind a  \eqdef (R_1@\elind a,\ldots,R_k@\elind a)
            \end{align*}
            is defined, and it satisfies $R$ in the structure $B_{\elind a}$.  Once we have defined these formulas, the claim will follow, by taking the disjunction over all finitely many possible grade profiles.
            

            Let then $\pi$ be a grade profile $\pi$ and relation name $R$. Suppose that we are given elements $\bar c$ and $a$ such that $\bar c@\elind a$ is entirely defined and has grade profile $\pi$. All of this can be checked in \mso. We want to know if the relation $R$ is satisfied in $B_{\elind a}$. 
            Let $i \le \elind a$ be the minimal index that  the entire tuple $\bar c@i$  is  defined. By minimality, we know that at least coordinate in the tuple  $\bar c@i$ is down-graded. In the first step, we will apply the induction assumption on profiles (and the fact that some coordinate in $\bar c@i$ is down-graded) to  prove that we can compute in \mso  the quantifier-free theory of $\bar c@i$ inside $B_i$.
        In the second step, we will this theory to compute the  quantifier-free theory of $\bar c @ \elind a$ in $B_{\elind a}$, which will tell us if the predicate $R$ is satisfied. 

        \begin{enumerate}
            \item We begin by computing the quantifier-free theory
            \begin{align*}
            \theory_0(B_i, \bar c@i).
            \end{align*}
            If $i=1$, then there is nothing to do, since we can simply use the already known structure $\chalf$ which contains all of $B_1$. Assume then that $i > 1$. Let $R_1,\ldots,R_k$ be the coordinates of $\bar c$.  Each  such  coordinate $R_j$  has origin of the form $q_j(\bar d_j)$ for some component $q_j$ of the state update function and some tuple $\bar d_j$ of elements of index $i-1$. 
              The important thing is that the profile of $\bar d$ is strictly smaller than the profile of $\bar c$, because we have chosen $i$ so that at least one coordinate $R_j@i$ is down-graded. 
              The components $q_1,\ldots,q_k$ and the tuple $\bar d = \bar d_1 \cdots \bar d_k$  can be found in \mso using the structure $\chalf$. Because the state update function is graded polyregular, once the components $q_1,\ldots,q_k$ are known, the quantifier-free theory of $\bar c@i$ in $B_i$  is uniquely determined by the quantifier-free theory 
              \begin{align*}
              \theory_0((B_{i-1},A_{i-1}),\bar d)
              \end{align*}
              and the  \mso theory 
              \begin{align*}
                \theory_r(((B_{i-1},A_{i-1}),\bar d)|\ell+1)
                \end{align*}
              for some quantifier rank $r$ that depends only on the state update function. The  \mso theory can be computed in \mso inside the structure $\chalf$ which is part of the input, since it concerns only elements of grade at least $\ell+1$. By compositionality, the quantifier-free theory is uniquely determined by the quantifier-free theories 
              \begin{align*}
                \theory_0(B_{i-1},\bar d \cap B_{i-1})
                \qquad 
                \theory_0(A_{i-1},\bar d \cap A_{i-1}).
                \end{align*}
            The latter theory is given in the input structure, while the former theory can be computed by induction assumption on a smaller grade profile.

              \item We now use the quantifier-free theory from the previous item to compute the theories  
              \begin{align*}
              \theory_0(B_j, \bar c @j) \qquad \text{for $j \in \set{i,\ldots,\elind a}$.}
              \end{align*}
              Using the same argument as in Claim~\ref{claim:at-defined}, we can show that for every  $j \in \set{i,\ldots \elind a-1}$, one can compute in \mso over $\chalf$  a partial  transformation  on quantifier-free theories which implements 
              \begin{align*}
                \theory_0(B_j, \bar c @j) \quad \mapsto \quad  \theory_0(B_{j+1}, \bar c @(j+1) ).
                \end{align*}
              By composing these transformations for all $j \in \set{i, \ldots, \elind a -1}$, and then applying the resulting transformation to the theory from the previous item, we can get the desired quantifier-free theory 
              \begin{align*}
              \theory_0(B_{\elind a}, \bar c @ \elind a.)
              \end{align*}
        \end{enumerate}
        
    \end{proof}
    
\end{proof}

==> origins.tex <==
\section{Origins}

\nocite{bojanczykTransducersOriginInformation2014}


Consider an infinite set $\atoms$, whose elements will be called \emph{atoms}, and used as identifiers for positions. A \emph{linear original function} is a function of type 
\begin{align*}
f : (\Sigma \times \atoms)^+ \to (\Gamma \times \atoms)^+
\end{align*}
which commutes with every atom renaming, in the sense that for every function $\pi : \atoms \to \atoms$, which need not be a permutation, the following diagram commutes: 



\subsection{Polyregular origins}


\begin{theorem}
    Consider an original function 
    \begin{align*}
        f : (\Sigma \times \atoms)^+ \to (\Gamma \times \atoms^{\le k})^+.
        \end{align*}
    
    \begin{enumerate}
        \item Then $f$ is definable by an \mso interpretation if: 
        \begin{enumerate}
            \item there is some bound $m \in \set{0,1,\ldots}$ such that for every input $w$ with unique, the output $f(w)$ contains each tuple of atoms at most $m$ times; and 
        \end{enumerate}
    \end{enumerate}
\end{theorem}

==> polyregular-are-derivable.tex <==
\subsection{Polyregular functions are weakly derivable}
We begin by proving the left-to-right implication in Theorem~\ref{thm:main}, which says that every polyregular function between two non-graded datatypes  is weakly derivable.


The proof is by decomposing the polyregular function into simpler functions, and weakly deriving the simpler function. This strategy works because of the following observation.

\begin{lemma}\label{lem:weakly-derivable-composition}
    Weakly derivable functions are closed under composition.
\end{lemma}
\begin{proof}
    Thanks to functoriality of bind and composition of functions we can derive the following rule
    \begin{align*}
        \frac{ \upgrade \tau_k \to \sigma \quad \upgrade \sigma_\ell \to \pi}{ \upgrade{\tau}_{k + \ell} \to \pi }.
    \end{align*}
\end{proof}

The next step is to reduce the problem to string-to-string functions. We will do this by representing non-graded datatypes using strings over a fixed finite alphabet in the obvious way.  

\begin{lemma}Let $\sigma$ be the finite alphabet consisting of letters
    \begin{align*}
        [\quad ] \quad ( \quad ) \quad , \quad \leftinj \quad \rightinj \quad 1,
    \end{align*}
    viewed as a non-graded datatype using co-product representation.
    For every non-graded datatype  $\tau$  there are functions 
    \[
    \begin{tikzcd}[column sep = 2cm]
    \tau 
    \ar[r,"\savefun", bend left=20]
    &
    \sigma^+
    \ar[l,"\loadfun", bend left=20]
    \end{tikzcd}
    \]
    which are both  weakly derivable and polyregular, and such that $\savefun;\loadfun$ is the identity on $\tau$. 
\end{lemma}
\begin{proof}
    The functions are the obvious way of writing an element of a datatype as a string. For example, if the datatype  is
\begin{align*}
\tau = {(1 + 1)^+} \times (1 \times 1)^+
\end{align*} 
then an element of $\tau$ can be seen as a string in $\sigma^+$ like this:
\begin{align*}
([\leftinj 1, \rightinj 1, \leftinj 1], [(1,1),(1,1),(1,1)]).
\end{align*}
The function $\loadfun$ needs to account for ill-formatted strings, i.e.~strings that are not in the range of the function $\savefun$. This is solved by mapping all  ill-formatted strings to some fixed element of $\tau$.  The $\savefun$ function can even be derived 
Note that although the datatype uses strengthening $\upgrade{ \ }$, this is not reflected in the element, since the set represented by a datatype ignores strengthening.
The \emph{string representation} of the element is defined to be string, as in~\eqref{eq:string-representation}, which is used to write down the element, and which uses the finite alphabet

\end{proof}


Thanks to the above two lemmas, in order to show that every polyregular function between datatypes is weakly derivable, it is enough to prove this only for polyregular string-to-string functions. Indeed, suppose that $f : \tau \to \rho$ is polyregular. Consider the following diagram:
\[
\begin{tikzcd}[column sep=2cm]
    \sigma^+ 
    \ar[r,"\loadfun_\tau", bend left=20]
    &
    \tau
    \ar[l,"\savefun_\tau", bend left=20]
\ar[r,"f"]
& 
\rho
    \ar[r,"\savefun_\rho", bend left=20]
    &
    \sigma^+
    \ar[l,"\loadfun_\rho", bend left=20]
\end{tikzcd}
\]
Since polyregular functions are closed under composition, and both $\loadfun$ and $\savefun$ are polyregular, it follows that the function 
\begin{align*}
  \loadfun_\tau\ ;\  f\ ;\  \savefun_\rho,
\end{align*}
which describes the path from left to right in the above diagram, is polyregular. Therefore, if we know that all polyregular string-to-string functions are weakly derivable, then this function would be weakly derivable. Therefore, also 
\begin{align*}
    \myunderbrace{\savefun_\tau \ ;\ \loadfun_\tau\ ;\  f\ ;\  \savefun_\rho \ ;\  \loadfun_\rho}{this is the same as $f$}
  \end{align*}
  would also be weakly derivable, since weakly derivable functions are closed under composition and contain both the $\savefun$ and $\loadfun$ functions.

  Therefore, it remains to show that all polyregular string-to-string functions are weakly derivable. These can be further decomposed: as shown in~\cite[Theorem 4.4]{bojanczykPolyregularFunctions2018}, every polyregular string-to-string function can be decomposed as a finite compositions which are either regular, or are the  \emph{square underline} function of type 
  \begin{align*}
  \tau^+ \to (\tau+\tau)^+
  \end{align*}
  which is explained in the following example: 
    \begin{align*}
    abcd \quad \mapsto \quad \myunderbrace{\underline abcd \  a\underline bcd\  ab \underline cd\ abc\underline d}{the non-underlined letters are from the first copy of $\tau$ \\ 
    \scriptsize and the underlined letters are from the second copy of $\tau$}.
    \end{align*}
    Formally speaking, the square underline is not one function, but a family of functions indexed by the input alphabet $\tau$ (in fact, it would be enough to use only the case of $\tau$ being a two-letter alphabet, but this will not be helpful anyway). Therefore, it is going to be enough to show that the square underline function is derivable, and also every regular string-to-string function is derivable. 


\begin{lemma} \label{lem:regular-weakly-derviable}  If $\tau$ and $\sigma$ are finite sets, viewed as datatypes in co-product representation, then every function  $f : \tau^+ \to \sigma^+$  computed by a streaming string transducer is weakly derivable. \end{lemma}
\begin{proof}

Define a \emph{register update} to be a function of type 
\begin{align*}
(\Gamma^+)^k \to (\Gamma^+)^\ell \qquad \text{with $k, \ell \in \set{0,1,\ldots}$}
\end{align*}
which has the following form. The function is given by $\ell$  words 
\begin{align}\label{eq:strings-defining-a-register-update}
w_1,\ldots,w_\ell \in (\Gamma + \set{1,\ldots,k})^k.
\end{align} 
Using these words, the register update  is defined as follows: given an input register valuation in $(\Gamma^+)^k$, the  output register valuation in $(\Gamma^+)^\ell$  is obtained by taking the words $w_1,\ldots,w_\ell$, and replacing each letter $i \in \set{1,\ldots,k}$ with the contents of the $i$-th register in the input register valuation. A register update is called \emph{copy-less} if every letter from $\set{1,\ldots,k}$ appears in at most one of the strings from~\eqref{eq:strings-defining-a-register-update}, and it appears at most once in that string. 


A streaming string transducer is defined as follows. There is an input alphabet $\Sigma$, an output alphabet $\Gamma$, a set states $Q$, with designated initial state. There is a state update function 
\begin{align*}
\delta : Q \times \Sigma \to Q
\end{align*}
as in a deterministic finite automaton. There is a number of registers $k \in \set{0,1,\ldots}$, and for  every state $q$ there is a copy-less register update function 
\begin{align*}
\gamma_q : (\Gamma^k)^+ \to (\Gamma^k)^+.
\end{align*}
Finally, there is an output copy-less register update 
\begin{align*}
out : (\Gamma^k)^+ \to \Gamma^+.
\end{align*}
The semantics of the automaton is defined as follows. A configuration consists of a state and a register valuation in $(\Gamma^+)^k$. The initial configuration use the initial state and the register valuation where all registers are empty. When reading an input letter $a \in \Gamma$, the configuration is updated as follows: the state is updated using the state update function, and then the register update function corresponding to the new state is applied to the register valuation. The output string is produced by applying the output register update to the register valuation in the last configuration, the one after reading all input letters. 

    We will derive the function 
    \begin{align*}
        \upgrade f:  \upgrade{\tau^+}_2 \to \sigma^+.
    \end{align*}
Consider the configuration space of the automaton. We can view this space as a co-product of several copies of the set $(\Gamma^+)^k$ of register valuations, with one copy for every control state:
\begin{align*}
\tau = \coprod_{q \in Q} (\Gamma^+)^k.
\end{align*}
Taking this view, the transition function of the sst can be seen as a function of  type 
\begin{align*}
\delta :  \sigma \times \tau \to \tau.
\end{align*}
We will show that this function can be derived, assuming that the input letter is under the scope of the bind operation. 
\begin{claim}The function is derivable:
    \begin{align*}
    (\upgrade a, c) \in \upgrade \Sigma \times \tau 
    \qquad \mapsto \qquad 
    \delta(a,c) \in \tau.
    \end{align*}
\end{claim}
Before proving the claim, we use it to finish the proof of the lemma. By applying fold to the function from the claim, we can derive the function  of type
\begin{align*}
 \upgrade{\upgrade{\Sigma}^+} \to \tau
\end{align*}
which maps an input string to the register valuation after reading it (the input letters are strengthened by bind, and the entire list is also strengthened by bind). Since bind commutes with lists, the input type can be changed to the type required in the lemma, while the output can also be recovered by using the output function of the sst. It remains to prove the claim.

\begin{proof}
    Because bind commutes with co-product, we can derive a function of type 
    \begin{align*}
    \upgrade \Sigma \times \tau \quad \to \quad \coprod_{a \in \Sigma} \coprod_{q \in Q} \upgrade 1 \times (\Gamma^+)^k 
    \end{align*}
    which moves the co-product to the top level of the type. By functoriality of co-products, in order to finish the proof of the claim, it remains to show that for every copy-less register update 
    \begin{align*}
    \gamma : (\Gamma^+)^k \to (\Gamma^+)^k,
    \end{align*}
    one can derive the function 
    \begin{align}
        \label{eq:gamma-with-extra-seed}
    (\upgrade 1, v) \in \upgrade 1 \times (\Gamma^+)^k 
    \quad \mapsto \quad \gamma(v) \in (\Gamma^+)^k, 
    \end{align}
    which works the same way as $\gamma$, except that it uses an extra argument of type $\upgrade 1$. The idea is that the extra argument is used to generate the new letters that are created during the register update.  We show how to derive the function from~\eqref{eq:gamma-with-extra-seed} on an example, where $k=3$ and the register update is 
    \begin{align*}
    (A,B,C) \qquad \mapsto \qquad (\varepsilon, AaCb, aB) 
    \end{align*}
    This register update is derived in the following diagram:
    \mypic{1}
\end{proof} 
\end{proof}



    \begin{lemma}\label{lem:square-underline}
        For every datatype $\tau$, the  square underline function for alphabet $\tau$ is weakly derivable.
    \end{lemma}
    \begin{proof}

        \begin{enumerate}
            \item In the first step, we show that  we can can weakly derive the function which maps a list to all of its non-empty prefixes, as in the following example:
            \begin{align*}
                [1,2,3] \quad \mapsto \quad  [[1],[1,2],[1,2,3]].
                \end{align*}
                Assuming that the list elements have type $\sigma$, we will derive this function in type 
                \begin{align*}
                \upgrade{\sigma^+}_2 \to \sigma^{**}.
                \end{align*}
            We will use fold for the following automaton.  The input alphabet of the underlying automaton is $\upgrade \sigma$, and its   state space is
            \begin{align*}
            \tau = \sigma^{**} \times \upgrade{\sigma^+}.
            \end{align*}
            The idea is that the first coordinate stores the list of prefixes, and the second coordinate stores the input list. The initial state is the pair of empty lists, in type $\tau$. 
            The transition function of the automaton  is
            derived in the following diagram:
            \mypic{3}
            By applying fold to the automaton defined above, we derive prefixes function in type 
            \begin{align*}
            \upgrade{ \upgrade{\sigma}^+} \to \sigma^{**}.
            \end{align*}
            Since strengthening commutes with lists, the above function can be also derived in type 
            \begin{align*}
            \upgrade{\sigma^+}_2 \to \sigma^{**},
            \end{align*}
            i.e.~the prefixes function can be weakly derived.
            \item In the second step, we apply the prefixes function, then the reverse function, and then the prefixes function again. The composition of these three functions  is the function of type $\sigma \to \sigma^{***}$ that is  illustrated in the following example:
            \begin{gather*}
                [1,2,3] \\ \downmapsto \\  [[[1,2,3]], [[1,2,3],[1,2]], [[1,2,3],[1,2],[1]]]
            \end{gather*}
            This function can be weakly derived, by the previous item, Example~\ref{ex:reverse-derivable}, and closure of weakly derivable functions under composition.
            \item From the output of the function in the previous item, we can extract the square underline using a regular function. Indeed, if the input list to the function in the previous item is  $[a_1,\ldots,a_n]$, then the $i$-th list in the output list has the form 
            \begin{align*}
            [[a_1,\ldots,a_n],[a_1,\ldots,a_{n-1}],\ldots,[a_1,\ldots,a_i]].
            \end{align*}
            To get the $i$-th part of the square underline, we should output the last list (with its last element underlined), followed by the last elements of the remaining lists, in opposite order. This is an example of a regular string-to-string transformation, and thus it is weakly derivable.
        \end{enumerate}
    \end{proof}

  






==> rubbish.tex <==



\subsection{Derivable functions}
We now present the central definition of this paper: the derivable  functions. These are functions between graded datatypes, i.e.~datatypes that can use  add the upgrade constructor $\upgrade \tau$ as well as the standard constructors of products, co-products and lists. The functions transform  graded structures. We keep all of the prime functions and combinators for quantifier-free functions from Theorem~\ref{thm:fold-quantifier-free} (but these now range over graded datatypes), and  we add several new ones that deal with the grades. The new prime functions are 
\begin{align*}
\primepoly
\end{align*}
The important new prime function is copying. It says that we can freely create  downgraded copies.  The new combinators are 
\begin{align*}
\combpoly
\end{align*}
For convenience, all prime functions and combinators are collected in Figures~\ref{fig:prime-poly} and~\ref{fig:comb-poly}.
\begin{definition}
    Let $\tau$ and $\sigma$ be graded datatypes. 
    A function $f : \tau \to \sigma$ is called \emph{derivable} if it can be obtained using the prime functions in Figure~\ref{fig:prime-poly} by applying the combinators in Figure~\ref{fig:comb-poly}.
\end{definition}


\begin{figure}
    \begin{align*}
        \primepr\\
        \primepoly
    \end{align*}
    \caption{\label{fig:prime-poly} The prime derivable functions}
\end{figure}

\begin{figure}
    \begin{align*}
        \combqf 
        % \combpoly
    \end{align*}
    \caption{\label{fig:comb-poly} The combinators for derivable functions}
\end{figure}



% \begin{myexample}\label{ex:identity}
%     Let us first show that for every graded datatype $\tau$, the identity function $\tau \to \tau$ can be derived. This is proved by induction on the datatype: for the datatype $1 \to 1$ the identity is one of the prime functions, while for more complicated types we use the functoriality combinators. 
% \end{myexample}

To avoid confusion, from now on we use the name \emph{non-graded datatype} for datatypes without the upgrade constructor, and we never speak of datatypes without specifying if they are graded or non-graded. Non-graded datatypes can be seen as a special case of graded ones, in the corresponding structures all elements have grade zero. 
We are now ready to state our main theorem, which says that the polyregular functions are exactly the derivable ones, as long as we allow the argument to be upgraded a fixed number of times. The theorem is stated for non-graded datatypes, because so far we have notion of polyregular function only for non-graded datatypes. 


    











\begin{myexample}\label{ex:finite-automata} 
    Consider a finite alphabet $\sigma$, viewed as a datatype using co-product representation, and a regular language over this alphabet. The language can be viewed as a function 
    \begin{align*}
    L : \sigma^+ \to \myunderbrace{\set{\text{yes, no}}}{$1 + 1$}.
    \end{align*}
    We will show that this function is  derivable in type 
    \begin{align*}
    \upgradelong{\sigma^+} \to \set{\text{yes, no}}.
    \end{align*}
    The idea is to take a deterministic finite automaton that recognizes $L$, and to evaluate it using the fold operator.  More precisely, consider a deterministic finite automaton $\Aa$ that recognizes the language, which has state space $Q$. We think of $Q$ as being a datatype, using the co-product representation. Consider the function 
    \begin{align*}
    \delta : (1 + Q \times \Sigma) \to Q
    \end{align*}
    which represents the initial state and transition function of the automaton. This function is derivable, in its original type: by using  distributivity, we can convert the input into the co-product representation of the set $1 + Q  \times \sigma$, and then use  Example~\ref{ex:finite-sets}. By applying fold to $\delta$ we can derive the function 
    \begin{align*}
    \delta^+ : \upgradelong{\sigma^+} \to Q
    \end{align*}
    which maps a word to the state after reading it; and then we can compose the result with the acceptance criterion of the automaton
    \begin{align*}
    F : Q \to \set{\text{yes,no}}.
    \end{align*}
\end{myexample}




\begin{lemma}
    If the fold combinator is applied to a copyless \mso interpretation, then it yields a copyless \mso interpretation.
\end{lemma}
\begin{proof}
    Consider a copyless \mso interpretation 
    \begin{align*}
     f : \underline{(1 + \sigma \times \tau)} \to \underline{\tau}.
    \end{align*}
    This interpretation is given by a universe formula, and a family of formulas indexed by the relations in the vocabulary of $\underline \tau$. Let $k \in \set{0,1,\ldots}$ be the maximal quantifier grade of the formulas used in the definition of $ f$. For a model 


    \begin{align*}
    [M_1,\ldots,M_n] \in \underline{\tau^+}.
    \end{align*}
\end{proof}



\begin{lemma}
    Every polyregular function is derivable in type 
\end{lemma}

\begin{lemma}
    Let $f : \Sigma^+ \to \Gamma^+$ be a string-to-string function, for finite alphabets $\Sigma$ and $\Gamma$. We view the two alphabets as types using the the co-product representation from Example~\ref{ex:finite-sets}. Then 
    \begin{enumerate}
        \item if $f$ is linear regular then it is derivable without using the function $\upgrade \tau \to \upgrade \tau \times \tau$;
        \item if $f$ is polyregular, then it is derivable.
    \end{enumerate}
\end{lemma}
\begin{proof}
    
    \paragraph*{Step 1.} A \emph{Mealy machine} is a deterministic finite automaton with transitions labelled by output letters. The semantics of a Mealy machine is a letter-to-letter function of type $\Sigma^+ \to \Gamma^+$, where $\Sigma$ is the input alphabet and $\Gamma$ is the output alphabet.  The first observation is that every function computed by a Mealy machine is derivable. Indeed, we consider the set 
    \begin{align*}
    \tau = \coprod_{q \in Q} \Gamma^+,
    \end{align*}
    which is a disjoint union of finitely many copies of $\Gamma^+$, with one copy for every state $q \in Q$ of the Mealy machine. We will think of an element of $\tau$ as consisting of an output string, together with a colour that is a state. Consider the function 
    \begin{align*}
    \delta : (1 + \tau \times \Sigma) \to \tau
    \end{align*}
    which is defined as follows. If the input is in $1$, then the output is the empty output string, coloured by the initial state. Otherwise, if the input is an output string $w \in \Gamma^+$ coloured by some state $q$, and an input letter $a \in \Sigma$  then the output is obtained as follows: apply the transition function  of the Mealy machine to $q$ and $a$, yielding a pair consisting of a new state $p$ and an output letter $b$, and return the list $wb$ coloured by the state $b$. 
    \begin{claim}  
        The function $\delta$ is derivable.
    \end{claim}
    If we apply the fold combinator to $\delta$, then we get the function of type $\Sigma^+ \to \Gamma^+$ that is computed by the Mealy machine. 

    \paragraph*{Step 2. Reverse.} Consider the reverse function. This function is derivable. Indeed, we can apply the fold combinator to the function 
    \begin{align*}
    1 + (\tau^+ \times \tau) \to \tau^+
    \end{align*}
    which returns the empty list on input from $1$, and otherwise prepends the argument from $\tau$ to the argument from $\tau^+$. The result is list reversal.

    \paragraph*{Step 3. \mso relabelling.} Consider an \mso formula $\varphi(x)$ with one free first-order variable, which describes a property 

    \begin{align*}
    \Sigma \times \coprod_{q \in Q} \Gamma^+ \to \coprod_{\substack{q \in Q \\ a \in \Sigma}} 1 \times \Gamma^+
    \end{align*}
    transition function of the Mealy machine 
    \begin{align*}
    \delta : (Q \times \Sigma) \to (Q \times \Gamma)
    \end{align*}

\end{proof}
\begin{lemma}
    If a function $f : \Sigma^+ \to \Gamma^+$ is computed by a Mealy machine, then it is derivable. 
\end{lemma}


\begin{theorem} \label{thm:main} Let $\tau$ and $\sigma$ be non-graded datatypes.  A function  $f : \tau \to \sigma$ is polyregular if and only if there is some $n \in \set{0,1,\ldots}$ such that one  can derive the function 
\begin{align*}
\myunderbrace{\upgraden x n \in \upgraden \tau n}{$\upgraden x n$ is $x$ upgraded $n$ times} \qquad \mapsto \qquad f(x) \in \sigma.
\end{align*}    
\end{theorem}

In the proof below, we will say that a function is \emph{weakly derivable} if it satisfies the second condition in the equivalence from the above theorem, i.e.~it can be derived after upgrading the argument some fixed number of times. In this terminology, the above theorem says that the polyregular functions are exactly the weakly derivable functions. 

In principle, we care about weakly derivable functions between non-graded datatypes, but the notion also applies to functions between graded datatypes. For example, the  function 
\begin{align*}
\upgrade 1 \in \upgrade 1 \qquad \mapsto \qquad (\upgrade 1, \upgrade 1) \in \upgrade 1 \times \upgrade 1
\end{align*}
is not derivable but weakly derivable, since one can derive 
\begin{align*}
    \upgraden 1 2 \in \upgraden 1 2 \qquad \mapsto \qquad (\upgrade 1, \upgrade 1) \in \upgrade 1 \times \upgrade 1
    \end{align*}
by using copying.



In the system without fold, an important function will be the split function of type 
\begin{align*}
\Sigma^*  \to \Sigma^* \times \Sigma^*
\end{align*}
which  outputs all possible ways of splitting the input list into (prefix, suffix) pairs, as explained in the following example:
\begin{gather*}
[1,2,3] \\ \downmapsto \\ [([],[1,2,3]),([1],[2,3]),([1,2],[3]),([1,2,3],[])].
\end{gather*}
The completeness result for the system without fold is stated in the following theorem, which was proved in~\cite[p.~64]{bojanczykPolyregularFunctions2018} adjusting for slightly different notation

In this paper, we mainly focus on a description of the polyregular functions that uses certain atomic functions, such as string concatenation, and combines them using certain combinators, such as a function composition. For this approach, it is more convenient to work with types that have more structure than simple strings, e.g.~we want to have pairs, or pairs of lists, or lists of lists, etc. The types used are described in the following definition. 
\begin{definition}
    A \emph{string type} is any type that is constructed using the following type constructors
    \begin{align*}
        \myunderbrace{1}{a type with \\ \scriptsize  one element} \qquad 
        \myunderbrace{\Sigma_1 \times \Sigma_2}{pair} \qquad \myunderbrace{\Sigma_1 + \Sigma_2}{co-pair, i.e.\\ \scriptsize disjoint union} \qquad \myunderbrace{\Sigma^*}{lists}.
        \end{align*}
\end{definition}

The set of strings over any finite alphabet can be seen as a string type: namely strings over an alphabet with $n$ letters are viewed as the type
\begin{align}\label{eq:type-of-strings}
(\myunderbrace{1+ \cdots + 1}{$n$ times})^*.
\end{align}
Ultimately, we will be interested in functions where both the input and output types are as in~\eqref{eq:type-of-strings}. The purpose of the other string types will be to define intermediate functions.

The notion of polyregular function can easily be extended to functions where the input and output sets are  string types. One way to do this is to represent elements of string types as strings, and then use the usual notion of polyregular functions on strings. For example, an element of the type
\begin{align*}
((1+1)^* \times 1^*)^*.
\end{align*}
can be represented as a string
\begin{align*}
([\myunderbrace{\leftinj \myoverbrace{()}{the unique element of the type $1$}}{$\leftinj$ is the co-projection\\ of type $1 \to 1 + 1$}, \rightinj (), \leftinj ()], [(),(),()])
\end{align*}
over an alphabet that has seven letters: opening and closing brackets of the two kinds, the comma, and the two co-projections.
Using this representation, which we call \emph{serialization}, we can define a polyregular function between two string types to be any function that becomes polyregular when the inputs and outputs are represented using serialization. 

However, 
the purpose of string types is not to be converted back to strings using serialization.

When representing  string type as a class of structures, we will be rather careful about the vocabulary, because we will be interested in quantifier-free interpretations, and in this case the choice of vocabulary is important. In the definition below, we use a disjoint union operation on structures that is defined as follows. Consider two structures $A_1$ and $A_2$, in which the vocabularies need not be disjoint.  In the disjoint union, the universe is the disjoint union of the two universes, and the vocabulary is the non-disjoint union of the two vocabularies.  A relation name symbol $R$ is interpreted as the union, ranging over $i \in \set{1,2}$ such that $R$ is in the vocabulary of $A_i$, of those tuples in $A_i$ that satisfy the relation. Under this definition, the Boolean predicates, i.e.~the relations of arity zero, get aggregated using disjunction; but we will prefer to avoid this hack by taking disjoint unions of structures whose vocabularies are disjoint for  Boolean predicates.


% An element of a type $\Sigma$ can be visualized as a node-labelled, sibling-ordered tree, as illustrated in the following example:

% For a tree, we define its \emph{model} to be the following relational structure. The universe is the nodes of the tree. For every label there is a unary predicate $a(x)$ which is true in nodes with label $x$. There are also three functions: the parent function, the left-most child function, the right-most function. 

    We begin by commenting on the asymmetry between the first-to-last and last-to-first traversals of a list. In our system, the fold operation is applied in first-to-last order, which corresponds to the \emph{fold left} operation in Haskell. The prime function for list construction is compatible with the left fold, because it constructs the list in the same way as fold deconstructs it, namely beginning with the leftmost element. If we replaced the prime function 
    From the list constructor, we can easily derive a prepending function 
    \begin{align*}
    \primefunction{\Sigma \times \Sigma^*}{\to}{\Sigma^*}{prepend}
    \end{align*}
    In the proof below, it would be convenient to use a symmetric append function. However, to derive append, we would need to use list reversal, which is requires updating, and thus append can only be derived in type 
    \begin{align*}
    \Sigma \times !\Sigma^* \to \Sigma^*
    \end{align*} 


\newcommand{\submodel}[2]{#1|\text{(#2)}}

We begin by introducing some notation. Consider some input to the fold function 
\begin{align*}
(Q_0, [A_1,\ldots,A_n])\in \tau \times \sigma^*.
\end{align*}
In the proof below, when speaking of the input, we mean the above. We will use automata terminology in the proof, i.e.~we will refer to $Q_0$ as the \emph{initial state}, and we will use the name \emph{input letters} for the structures $A_1,\ldots,A_n$. 
For $i \in \set{1,\ldots,n}$, define $Q_i \in \tau$ to be the state of the automaton after reading the first $i$ letters, i.e. 
\begin{align*}
Q_{i} = \delta(Q_{i-1},A_{i}).
\end{align*}
The output of the fold function is the last state  $Q_n$, but in order to compute it, we will actually compute all states $Q_1,\ldots,Q_n$. 

Define a \emph{state element} to be an element of the universe in one of the state structures $Q_0,\ldots,Q_n$. We will also be interested in a \emph{parent function}, which is a partial function that maps  state elements from $Q_{i}$ to possibly undefined state elements from $Q_{i-1}$, as described below.  When a state  $Q_i$ is produced by applying the transition function to the pair $(Q_{i-1},A_i)$, we can classify the elements in the universe of  $Q_i$ into two kinds:
\begin{itemize}
\item equi-grade elements that belong to $Q_{i-1}$; and
\item the remaining elements, i.e.~down-graded elements, or equi-grade elements that belong to $A_i$.
\end{itemize}
For elements of the first kind, the \emph{parent} is defined to be the corresponding element in $Q_{i-1}$, and for elements of the second kind, the parent is undefined. 
% Let us write $Q^\ell_i$ for the elements of $Q_i$ that have grade $\ge \ell$ and origin exactly $i$, in other words they have grade $\ge \ell$ and kind (a). 
Define the \emph{run structure} to be the structure 
\begin{align*}
R = [Q_0,A_1,Q_1,\ldots, A_n,Q_n] \in (\tau + \sigma)^*
\end{align*}
together with the parent function. To prove the theorem, we will show  that the run structure can be computed by a graded polyregular function, in a way such that all state elements are down-graded. We will do this grade by grade, in the following sense. For a grade $\ell$, define \emph{grade $\ell$ run structure} $R_\ell$ to be the result of removing from the run structure the elements of $Q_1,\ldots,Q_n$ that have grade strictly smaller than  $\ell$. (All elements of $Q_0$ and $A_1,\ldots,A_n$ are kept, regardless of their grades.)  By induction on $\ell$, we will show that the grade $\ell$ run structure can be computed by a graded polyregular function. The induction is in the opposite order: the induction basis is when $\ell$ is one plus the maximal grade that appears in the input, and it proceeds down to $\ell=0$, in which case the run structure is obtained. In the induction basis there is nothing to do, since in this case the grade $\ell$ run structure contains no elements from $Q_1,\ldots,Q_n$. 

The rest of the proof is devoted to the induction step. Suppose that we already have the grade $\ell+1$ run structure, and we want to produce the grade $\ell$ run structure. 



For an element of $Q_i$ or $A_i$, the number $i$ is called its \emph{index}. 
For a state element, define its \emph{progenitor} to be the unique ancestor (i.e.~transitive reflexive closure of the parent relation) that has no parent. Since the parent function is injective (i.e.~there cannot be two state elements with the same parent), it follows that for every state element is represented uniquely by  is represent uniquely by its progenitor and its index. Therefore, we write $a@i$ for the at most one state element that has progenitor $a$ and index $i$. The element $a@i$ is undefined if there is no element in $Q_i$ that has progenitor $a$. We will also want to represent the index as an element of the run structure, and not as a number: to do this, we define the \emph{representation} of $i$ to be the unique king element of $A_i$. We overload the notation as follows: if $b$ is the representation of an index $i$, then we write $a@b$ as a synonym for $a@i$, otherwise $a@b$ is undefined. 

 We want this representation to be a pair of elements in the run structure, and therefore the index will be represented using the unique king element in the structure $A_i$. Summing up, the \emph{progenitor representation} of a state element from $Q_i$ is the pair (the progenitor, the king element of $A_i$). We write $a@b$ for the element which has progenitor representation $(a,b)$, this is element might not be defined, but if it is defined then it is unique. 

Consider a pair of elements $(a,b)$ in the run structure such that: (i) $a$ is a state element without a parent; and (ii)  $b$ is the king element of some $Q_i$ which contains an element with progenitor $a$. We  write $a@b$ for the unique element in $Q_i$ that has progenitor $a$. Otherwise $a@b$ is undefined, i.e.~it is undefined if either $a$ is not a state element without a parent, or 


the progenitor of $c$ and the 

For $i \in \set{1,\ldots,n}$, we define the \emph{representation of $i$} to be the element of the run structure which is the chosen element of $A_i$. Elements of  $Q_1,\ldots,Q_n$ in the run structure are called \emph{state elements}, the remaining elements of the run structure are called \emph{input elements}. The following notation will be key: the representation of state element $c$ in the run structure is the pair $(a,b)$ such that $a$ is a state element with no parent, $b$ is the representation of an index 

 






Let us define $Q^\ell_i$ to be the result of restricting the structure $Q_i$ to elements which either: (a) have grade $>\ell$; or (b) have grade exactly $\ell$ and no parent. The following claim shows that these structures can be computed, using \mso interpretations, based on the available information:



\begin{claim}
    There is an \mso formula $\varphi(x,y)$ such that for every input to the fold,
    \begin{align*}
    R_{\ell + 1} \models \varphi(a,b) \qquad \text{iff} \qquad \text{$a@b$ is defined}.
    \end{align*}
    \end{claim}


\begin{claim} Let $\psi(x_1,\ldots,x_k)$ be an \mso formula over the vocabulary of $\tau$.  
    There is an \mso formula $\varphi(x_1,\ldots,x_k,y)$ such that for every input to the fold,
    \begin{align*}
    R_{\ell + 1} \models \varphi(a_1,\ldots,a_k,b)
    \end{align*}
    holds if and only if: $a_1@b, \ldots, a_k@b$ are all defined and 
    satisfy 
    \begin{align*}
    Q_b \models \varphi(a_1@b,\ldots,a_k@b)
    \end{align*}
\end{claim}


\begin{claim}\label{claim:equi-grade}
    There is an \mso interpretation
    \begin{align*}
    \gamma : \tau \times \sigma \to \tau,
    \end{align*}
     which depends only on $\ell$ and not the input, such that  
    \begin{align*}
    Q^\ell_i = \gamma(\submodel{(Q_{j-1},A_j)}{grade $> \ell$})
    \end{align*}
    holds for every input and every $i \in \set{1,\ldots,n}$. 
\end{claim}

\begin{claim}\label{claim:down-grade}
    For every $i \in \set{1,\ldots,n}$ there is a quantifier-free interpretation 
    \begin{align*}
    f_i : \tau \to \tau,
    \end{align*}
    which depends only on the quantifier-free theory of $A_i$, such that 
    \begin{align*}
    \submodel{Q_{i}} {origin $<i$} = f_i(\submodel{Q_{i-1}} {origin $<i$})
    \end{align*}
\end{claim}


By Claims~\ref{claim:equi-grade} and~\ref{claim:down-grade},  for every $j \le i \in \set{1,\ldots,n}$, we have
\begin{align*}
\submodel{Q_i}{origin $j$ and grade $\ge \ell$} =  \myunderbrace{f_{i} \circ f_{i-1} \circ \cdots \circ f_{j+1}}{call this $f_{ij}$}(Q^\ell_j).
\end{align*}
The function $f_{ij}$ belongs to the finite monoid of quantifier-free interpretations of type $\tau \to \tau$, and therefore similarly to Lemma~\ref{lem:}, it can be computed in \mso based on the indices $i$ and $j$ as well as the input $[A_1,\ldots,A_n]$. 
By induction assumption, the structure 
\begin{align*}
[Q_1^\ell, \ldots, Q_n^\ell]
\end{align*}
can be computed by an \mso interpretation.

To illustrate the main idea, we begin with a simpler special case of the lemma, which we call iteration.
    
\paragraph*{Iteration.}
For a function 
\begin{align*}
\delta : \Gamma \to \Gamma
\end{align*}
its iteration is defined to be the function 
\begin{align*}
\Gamma \times 1^* &\to \Gamma\\
(A,1^n) &\mapsto \delta^n(A).
\end{align*}
Iteration can be seen as the special case of fold where the function is not allowed to use the $\Sigma$ argument. The problems in Examples~\ref{ex:fold-duplication} and~\ref{ex:fold-tail} appeared already for iteration, so they must be addressed when proving the lemma for iteration.

To prove the lemma for iteration, we consider the monoid  $M$  of quantifier-free interpretations of type $\Gamma \to \Gamma$. This is a monoid, with the monoid operation being composition, since quantifier-free interpretations are closed under composition. Crucially, this monoid is finite, since there are finitely many quantifier-free formulas that can be written to define the universe and the relations.  The function 
\begin{align*}
1^n \quad \mapsto \quad f^n
\end{align*}
is a monoid homomorphism into a finite monoid, and therefore it is definable in \mso  in the sense that for every possible value $g \in M$ there is an \mso formula defining defining 
\begin{align*}
\setbuild { 1^n }{ $f^n = g$}.
\end{align*}
This completes the proof of the lemma: to compute the iteration on argument $(A,1^n)$, we first use an \mso formula evaluated in $1^n$ to compute the function $f^n$, and then we apply that function to $A$. 

\paragraph*{General case.}

We can even combine these functions into a quantifier-free interpretation 
\begin{align*}
1 + \tau \times \tau^+ \to \tau^+.
\end{align*}
This  is because quantifier-free interpretations can be combined using a ``cases'' combinator, as expressed by the rule 
\begin{align*}
    \frac{\tau_1 \to \sigma \quad \tau_2 \to \sigma}{\tau_1 + \tau_2 \to \sigma}.
\end{align*}
To see why quantifier-free interpretations are closed under this combinator, we define the universe formula to be 
\begin{align*}
\lor \begin{cases}
    R(x) \land \varphi_1(x) \\ \neg R(x) \land \varphi_2(x),
\end{cases}
\end{align*}
where $\varphi_i(x)$ is the universe formula for the $i$-th assumption of the ``cases'' rule.  Similarly, the formula defining  a predicate $P(x_1,\ldots,x_n)$ of the output vocabulary is 
\begin{align*}
    \lor \begin{cases}
        R(x_1) \land \cdots \land R(x_n) \land \varphi_{P,1}(x_1,\ldots,x_n) \\ \neg R(x_1) \land \cdots \land \neg R(x_n) \land \varphi_{P,1}(x_1,\ldots,x_n)
    \end{cases}
    \end{align*}
\begin{align*}
(\land_{i}R(x_i) \land \varphi_1(x_1,\ldots,x_n))
\end{align*}



Because $f$ is a quantifier-free interpretation, the elements of an output structure $f(A)$ a subset of the elements of the input structure $A$.  This motivates the following notation: for a structure $A \in \tau$, a tuple  $\bar a \in A^k$ of  distinguished elements, and a formula $\varphi$  with $k$ free variables, we write 
\begin{align}\label{eq:formula-after-interpretation}
f(A) \models \varphi(\bar a)
\end{align}
if all of the elements in the tuple $\bar a$ belong to the structure $f(A)$, and furthermore the formula $\varphi$ is satisfied. even if the formula $\varphi$ is ``true'', \eqref{eq:formula-after-interpretation} can fail; this will happen when some element of the tuple $\bar a$ is not defined in $f(A)$.    The following claim shows that quantifier-free formulas can be evaluated in $f^n(A, \bar a)$ by looking at \mso definable properties of $(A,1^n)$. 

\begin{claim}
    Let $\varphi$ be a  quantifier-free formula  over the vocabulary of $\tau$.   There is an \mso formula $\psi$ over the vocabulary of $\tau \times 1^*$, with the same number  of  free variables as $\varphi$, such that 
    \begin{align*}
       (A, 1^n) \models \psi(\bar a) \quad \text{iff} \quad f^n(A) \models \varphi(\bar a)
    \end{align*}
    holds for every $n \in \set{0,1,\ldots}$ and every  $A \in \tau$ with distinguished elements $\bar a$.
\end{claim}
\begin{proof}
    Let $k$ be the number of free variables in $\varphi$. 
    Suppose that $A$ and $B$ are structures in $\tau$, and each one comes with $k$ distinguished elements, denoted by $\bar a \in A^k$ and $\bar b \in B^k$. We write
    \begin{align*}
    A, \bar a \quad  \equiv \quad B, \bar b
    \end{align*}
    if the same quantifier-free formulas with $k$ variables are true on both sides.  Equivalence classes of $\equiv$ are called  \emph{quantifier-free type}.   We  will be interested in the quantifier-free type 
    \begin{align}\label{eq:qf-type-of-iteration}
        \typequot{(f^n(A), \bar a)},
        \end{align}
        which can be undefined if some distinguished element in $\bar a$ is not present in $f^n(A)$. We will show that this type 
    can be computed from the quantifier-free type of $A, \bar a$ and some \mso information about $n$.

    Because $f$ is a quantifier-free interpretation, it is a congruence with respect to quantifier-free types, in the following sense:  
\begin{align}\label{eq:congruence}
    A, \bar a \equiv B, \bar a\quad \text{implies} \quad 
    \myunderbrace{f(A), \bar a \equiv f(B), \bar a}{either both sides undefined, or \\ 
    \scriptsize both sides defined and equivalent}
    \end{align}
    This means that there is a well-defined partial function
    \begin{align*}
    \typequot{(A, \bar a)} \quad \mapsto \quad \typequot{(f(A, \bar a))},
    \end{align*}
    which inputs the quantifier-free type of a structure in $A$ with a tuple $\bar a$ of $k$ distinguished elements, and outputs the quantifier-free type of $f(A,\bar a)$, or an undefined value if the latter type is undefined. Let us write $\alpha$ for this partial function. Since $\alpha$ is a partial function from a finite set to itself (there are finitely many quantifier-free types once the vocabulary and number of free variables are fixed), the sequence of its powers 
    \begin{align*}
    \alpha^1, \alpha^2, \alpha^3, \ldots
    \end{align*} 
    uses finitely many distinct values and  is ultimately periodic. Since every ultimately periodic subset of $\setbuild{1^n}{$n \in \set{0,1,\ldots}$}$ is definable in \mso, it follows that  \mso can find the value of $\alpha^n$ based on the structure $1^n$. Since
    the quantifier-free type~\eqref{eq:qf-type-of-iteration}
    is obtained by applying $\alpha^n$ to  the quantifier-free type of $A,\bar a$, the  claim follows.
\end{proof}

From the claim we immediately get  the lemma. Apply the claim to the formula $\psi$ with one free variable that is equivalent to ``true'', yielding an \mso formula which selects those elements of $A$ that belong to the universe of  $f^n(A)$. Likewise, all of the relations in the structure $f^n(A)$, which are special cases of quantifier-free formulas, can be defined in \mso. Note that the \mso formulas are of a special form: they are Boolean combinations of quantifier-free formulas in $A$, and \mso formulas in $1^n$.  
